Effective Variable Depth Local Search for the Budgeted Maximum Coverage Problem

We address the Budgeted Maximum Coverage Problem (BMCP), which is a natural and more practical extension of the standard 0-1 knapsack problem and the set cover problem. Given m elements with nonnegative weights, n subsets of elements with nonnegative costs, and a total budget, BMCP aims to select some subsets such that the total cost of selected subsets does not exceed the budget, and the total weight of associated elements is maximized. In this paper, we propose a variable depth local search algorithm (VDLS) for the BMCP. VDLS first generates an initial solution by a greedy algorithm, then iteratively improves the solution through a partial depth-first search method, that can improve the solution by simultaneously changing the states (selected or not) of multiple subsets. Such method allows VDLS to explore the solution space widely and deeply, and to yield high-quality solutions. We further propose a neighbour structure to boost the algorithm performance, that is, both subsets have a neighbour relation if they have at least one common associated element. By applying the neighbour structure, VDLS can adjust the selected subsets while losing as few covered elements as possible. Since the existing BMCP benchmarks only have simple structures and small scales, we design 60 new instances with relatively large scales and complex structures to enrich the diversity of the BMCP instances. Experimental results on 30 public instances and 60 new instances we designed demonstrate that VDLS significantly outperforms the existing heuristic and the general CPLEX exact solver, for the BMCP.

==> table1-10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[b]
\centering
\caption{Comparison of the PLTS and VDLS with both 10 minutes of time limit, and the CPLEX solver with 2 hours and 5 hours of time limit in solving the 30 instances of the first set. Best results appear in bold.}
\label{table1-10}
\scalebox{0.56}{\begin{tabular}{lrrrrrrrrrrr} \toprule
\multirow{2}{*}{Instances} & \multicolumn{2}{r}{CPLEX(2 hours)}                         &                      & \multicolumn{2}{r}{CPLEX(5 hours)} &  & \multicolumn{2}{r}{PLTS}  &  & \multicolumn{2}{r}{VDLS}    \\ \cline{2-3} \cline{5-6} \cline{8-9} \cline{11-12} 
\multicolumn{1}{c}{}                           & LB                          & UB                           &                      & LB                  & UB           &  & best           & average  &  & best             & average  \\ \hline
bmcp\_585\_600\_0.05\_2000                     & 67910                       & 73495.9                      &                      & 70742               & 74224.9      &  & 70997          & 70892.6  &  & \textbf{71091}   & 71006.5  \\
bmcp\_585\_600\_0.075\_1500                    & 68418                       & 77549.4                      &                      & 69172               & 76716.9      &  & 70677          & 70535.9  &  & \textbf{71025}   & 70554.2  \\
bmcp\_600\_585\_0.05\_2000                     & 66184                       & 71739.7                      &                      & 66452               & 71094.3      &  & 67187          & 66807.1  &  & \textbf{67636}   & 67621.6  \\
bmcp\_600\_585\_0.075\_1500                    & 68145                       & 77321.5                      &                      & 70113               & 76332.9      &  & 70318          & 70318.0  &  & \textbf{70588}   & 70367.1  \\
bmcp\_600\_600\_0.05\_2000                     & 67917                       & 73495.1                      &                      & 68477               & 72880.9      &  & 68453          & 68346.6  &  & \textbf{68738}   & 68559.9  \\
bmcp\_600\_600\_0.075\_1500                    & 70947                       & 77380.0                      &                      & 71018               & 76337.7      &  & 71746          & 71746.0  &  & \textbf{71904}   & 71833.2  \\
bmcp\_685\_700\_0.05\_2000                     & 79997                       & 88954.3                      &                      & \textbf{80783}      & 88447.7      &  & 80111          & 79979.9  &  & 80751            & 80388.7  \\
bmcp\_685\_700\_0.075\_1500                    & 80443                       & 92328.3                      &                      & 81639               & 91379.0      &  & 82955          & 82933.4  &  & \textbf{83286}   & 82870.3  \\
bmcp\_700\_685\_0.05\_2000                     & 76139                       & 83561.9                      &                      & 77176               & 82815.1      &  & \textbf{78054} & 77460.8  &  & \textbf{78054}   & 77674.4  \\
bmcp\_700\_685\_0.075\_1500                    & 75841                       & 86956.9                      &                      & 76033               & 86566.8      &  & \textbf{78869} & 78580.1  &  & \textbf{78869}   & 78649.1  \\
bmcp\_700\_700\_0.05\_2000                     & 76367                       & 85587.3                      &                      & 77056               & 84855.4      &  & 77424          & 77225.8  &  & \textbf{78458}   & 78252.7  \\
bmcp\_700\_700\_0.075\_1500                    & 81645                       & 93026.7                      &                      & 81645               & 92152.0      &  & 84570          & 83406.5  &  & \textbf{84576}   & 84576.0  \\
bmcp\_785\_800\_0.05\_2000                     & 90705                       & 102198.7                     &                      & 91319               & 101585.7     &  & 92505          & 92080.7  &  & \textbf{92630}   & 92400.1  \\
bmcp\_785\_800\_0.075\_1500                    & 92358                       & 107354.5                     &                      & 92358               & 106842.7     &  & 94245          & 94243.8  &  & \textbf{95221}   & 95221.0  \\
bmcp\_800\_785\_0.05\_2000                     & 86139                       & 97891.1                      &                      & 86813               & 97477.3      &  & 88562          & 88424.3  &  & \textbf{89138}   & 89024.7  \\
bmcp\_800\_785\_0.075\_1500                    & 89018                       & 103644.1                     &                      & 89229               & 102868.0     &  & 91021          & 90888.9  &  & \textbf{91856}   & 91644.6  \\
bmcp\_800\_800\_0.05\_2000                     & 90344                       & 101141.0                     &                      & 89872               & 100373.8     &  & 90951          & 90697.4  &  & \textbf{91795}   & 91541.8  \\
bmcp\_800\_800\_0.075\_1500                    & 94049                       & 108713.0                     &                      & 94049               & 108005.6     &  & 95533          & 95508.8  &  & \textbf{95995}   & 95652.6  \\
bmcp\_885\_900\_0.05\_2000                     & 100085                      & 114313.8                     &                      & 99845               & 113747.0     &  & 101293         & 100857.0 &  & \textbf{102277}  & 101853.2 \\
bmcp\_885\_900\_0.075\_1500                    & 102423                      & 122684.4                     &                      & 102933              & 122093.5     &  & 105718         & 105707.7 &  & \textbf{106940}  & 106477.2 \\
bmcp\_900\_885\_0.05\_2000                     & 97088                       & 110828.8                     &                      & 96945               & 109948.5     &  & 98840          & 98485.5  &  & \textbf{99590}   & 99289.1  \\
bmcp\_900\_885\_0.075\_1500                    & 99881                       & 119045.5                     &                      & 99888               & 118554.8     &  & 103596         & 103223.1 &  & \textbf{105141}  & 104991.6 \\
bmcp\_900\_900\_0.05\_2000                     & 100108                      & 115682.6                     &                      & 100412              & 114551.1     &  & 101265         & 101210.7 &  & \textbf{101857}  & 101089.2 \\
bmcp\_900\_900\_0.075\_1500                    & 101035                      & 120452.8                     &                      & 99888               & 118554.8     &  & 104521         & 104521.0 &  & \textbf{105081}  & 104955.7 \\
bmcp\_985\_1000\_0.05\_2000                    & 107820                      & 125903.7                     &                      & 107488              & 124487.4     &  & 109523         & 108681.8 &  & \textbf{110319}  & 109673.1 \\
bmcp\_985\_1000\_0.075\_1500                   & 110769                      & 134440.4                     &                      & 111177              & 133789.8     &  & 113541         & 113439.4 &  & \textbf{115505}  & 115075.4 \\
bmcp\_1000\_985\_0.05\_2000                    & 108714                      & 126779.1                     &                      & 110134              & 125574.8     &  & 111212         & 110379.1 &  & \textbf{112057}  & 111552.3 \\
bmcp\_1000\_985\_0.075\_1500                   & 108801                      & 131873.0                     &                      & 108801              & 130981.4     &  & 112250         & 112160.2 &  & \textbf{113615}           & 112984.4 \\
bmcp\_1000\_1000\_0.05\_2000                   & 109928                      & 131194.2                     &                      & 111155              & 128583.6     &  & 111829         & 111318.6 &  & \textbf{113331}  & 113096.6 \\
bmcp\_1000\_1000\_0.075\_1500                  & 115313                      & 139152.9                     &                      & 115824     & 137900.4     &  & 118244         & 118243.1 &  & \textbf{120246}  & 119939.3 \\ \hline
Average                                        & \multicolumn{1}{l}{89484.4} & \multicolumn{1}{l}{103156.3} & \multicolumn{1}{l}{} & 89947.9             & 102324.1     &  & 91533.7        & 91276.8  &  & \textbf{92252.3} & 91960.5      \\ \bottomrule              
\end{tabular}}
\end{table}

==> table1-30.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\caption{Comparison of the PLTS and VDLS with both 30 minutes of time limit, and the CPLEX solver with 2 hours and 5 hours of time limit in solving the 30 instances of the first set. Best results appear in bold.}
\label{table1-30}
\scalebox{0.56}{\begin{tabular}{lrrrrrrrrrrr} \toprule
\multirow{2}{*}{Instances}    & \multicolumn{2}{r}{CPLEX(2 hours)} &  & \multicolumn{2}{r}{CPLEX(5 hours)} &  & \multicolumn{2}{r}{PLTS}   &  & \multicolumn{2}{r}{VDLS}    \\ \cline{2-3} \cline{5-6} \cline{8-9} \cline{11-12} 
                              & LB              & UB               &  & LB                  & UB           &  & best            & average  &  & best             & average  \\ \hline
bmcp\_585\_600\_0.05\_2000    & 67910           & 73495.9          &  & 70742               & 74224.9      &  & \textbf{71102}  & 70915.0  &  & 71091            & 71025.0  \\
bmcp\_585\_600\_0.075\_1500   & 68418           & 77549.4          &  & 69172               & 76716.9      &  & 70677           & 70670.2  &  & \textbf{71025}   & 70554.2  \\
bmcp\_600\_585\_0.05\_2000    & 66184           & 71739.7          &  & 66452               & 71094.3      &  & \textbf{67636}  & 67041.5  &  & \textbf{67636}   & 67621.6  \\
bmcp\_600\_585\_0.075\_1500   & 68145           & 77321.5          &  & 70113               & 76332.9      &  & 70318           & 70318.0  &  & \textbf{70588}   & 70371.7  \\
bmcp\_600\_600\_0.05\_2000    & 67917           & 73495.1          &  & 68477               & 72880.9      &  & 68453           & 68386.8  &  & \textbf{68738}   & 68620.1  \\
bmcp\_600\_600\_0.075\_1500   & 70947           & 77380.0          &  & 71018               & 76337.7      &  & 71746           & 71746.0  &  & \textbf{71904}   & 71833.2  \\
bmcp\_685\_700\_0.05\_2000    & 79997           & 88954.3          &  & 80783               & 88447.7      &  & 80197           & 80096.6  &  & \textbf{81227}   & 80551.6  \\
bmcp\_685\_700\_0.075\_1500   & 80443           & 92328.3          &  & 81639               & 91379.0      &  & 82955           & 82944.2  &  & \textbf{83286}   & 82870.3  \\
bmcp\_700\_685\_0.05\_2000    & 76139           & 83561.9          &  & 77176               & 82815.1      &  & 77876           & 77372.7  &  & \textbf{78054}   & 77780.5  \\
bmcp\_700\_685\_0.075\_1500   & 75841           & 86956.9          &  & 76033               & 86566.8      &  & \textbf{78869}  & 78810.4  &  & \textbf{78869}   & 78649.1  \\
bmcp\_700\_700\_0.05\_2000    & 76367           & 85587.3          &  & 77056               & 84855.4      &  & 78028           & 77501.5  &  & \textbf{78458}   & 78304.8  \\
bmcp\_700\_700\_0.075\_1500   & 81645           & 93026.7          &  & 81645               & 92152.0      &  & 84570           & 83720.7  &  & \textbf{84576}   & 84576.0  \\
bmcp\_785\_800\_0.05\_2000    & 90705           & 102198.7         &  & 91319               & 101585.7     &  & 92431           & 92195.7  &  & \textbf{92740}   & 92624.4  \\
bmcp\_785\_800\_0.075\_1500   & 92358           & 107354.5         &  & 92358               & 106842.7     &  & 94245           & 94245.0  &  & \textbf{95221}   & 95221.0  \\
bmcp\_800\_785\_0.05\_2000    & 86139           & 97891.1          &  & 86813               & 97477.3      &  & 88562           & 88560.3  &  & \textbf{89138}   & 89094.7  \\
bmcp\_800\_785\_0.075\_1500   & 89018           & 103644.1         &  & 89229               & 102868.0     &  & 91021           & 90971.8  &  & \textbf{91856}   & 91722.0  \\
bmcp\_800\_800\_0.05\_2000    & 90344           & 101141.0         &  & 89872               & 100373.8     &  & 91748           & 90934.2  &  & \textbf{91795}   & 91679.1  \\
bmcp\_800\_800\_0.075\_1500   & 94049           & 108713.0         &  & 94049               & 108005.6     &  & 95533           & 95533.0  &  & \textbf{95995}   & 95653.8  \\
bmcp\_885\_900\_0.05\_2000    & 100085          & 114313.8         &  & 99845               & 113747.0     &  & 101293          & 101142.0 &  & \textbf{102277}  & 102140.6 \\
bmcp\_885\_900\_0.075\_1500   & 102423          & 122684.4         &  & 102933              & 122093.5     &  & 106364          & 105782.6 &  & \textbf{106940}  & 106477.2 \\
bmcp\_900\_885\_0.05\_2000    & 97088           & 110828.8         &  & 96945               & 109948.5     &  & 98840           & 98645.4  &  & \textbf{99590}   & 99397.4  \\
bmcp\_900\_885\_0.075\_1500   & 99881           & 119045.5         &  & 99888               & 118554.8     &  & \textbf{105141} & 103846.9 &  & \textbf{105141}  & 104991.6 \\
bmcp\_900\_900\_0.05\_2000    & 100108          & 115682.6         &  & 100412              & 114551.1     &  & 101265          & 101211.4 &  & \textbf{102055}  & 101464.8 \\
bmcp\_900\_900\_0.075\_1500   & 101035          & 120452.8         &  & 99888               & 118554.8     &  & 104521          & 104521.0 &  & \textbf{105081}  & 104966.0 \\
bmcp\_985\_1000\_0.05\_2000   & 107820          & 125903.7         &  & 107488              & 124487.4     &  & 109567          & 108938.0 &  & \textbf{110669}  & 109868.9 \\
bmcp\_985\_1000\_0.075\_1500  & 110769          & 134440.4         &  & 111177              & 133789.8     &  & 113541          & 113541.0 &  & \textbf{115505}  & 115080.3 \\
bmcp\_1000\_985\_0.05\_2000   & 108714          & 126779.1         &  & 110134              & 125574.8     &  & 111176          & 110712.6 &  & \textbf{112057}  & 111849.7 \\
bmcp\_1000\_985\_0.075\_1500  & 108801          & 131873.0         &  & 108801              & 130981.4     &  & 112250          & 112218.9 &  & \textbf{113615}           & 113104.5 \\
bmcp\_1000\_1000\_0.05\_2000  & 109928          & 131194.2         &  & 111155              & 128583.6     &  & 112640          & 111577.8 &  & \textbf{113331}  & 113131.8 \\
bmcp\_1000\_1000\_0.075\_1500 & 115313          & 139152.9         &  & 115824     & 137900.4     &  & 119453          & 118499.3 &  & \textbf{120246}  & 119954.1 \\ \hline
Average                       & 89484.4         & 103156.3         &  & 89947.9             & 102324.1     &  & 91733.9         & 91420.0  &  & \textbf{92290.1} & 92039.3 \\ \bottomrule
\end{tabular}}
\end{table}

==> table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[b]
\centering
\caption{Comparison results of VDLS and PLTS, with 10 or 30 minutes of time limit, on the 30 instances of the second set. Best results appear in bold.}
\label{table2}
\scalebox{0.65}{\begin{tabular}{lrrrrr} \toprule
\multirow{2}{*}{Instances}  & \multicolumn{2}{r}{PLTS}   &  & \multicolumn{2}{r}{VDLS}     \\ \cline{2-3} \cline{5-6} 
                            & best            & average  &  & best              & average  \\ \hline
\multicolumn{6}{l}{10 minutes of time limit}                                               \\ \hline
bmcp\_1100\_1000\_0.3\_3000 & 142574          & 141985.1 &  & \textbf{143402}   & 142990.1 \\
bmcp\_1100\_1000\_0.5\_2000 & 125790          & 125479.5 &  & \textbf{126935}   & 126022.2 \\
bmcp\_1100\_1100\_0.3\_3000 & 154726          & 153867.0 &  & \textbf{157530}   & 156888.7 \\
bmcp\_1100\_1100\_0.5\_2000 & 138160          & 137490.0 &  & \textbf{139141}   & 138565.5 \\
bmcp\_1100\_1200\_0.3\_3000 & 169980          & 168661.8 &  & \textbf{172660}   & 171548.7 \\
bmcp\_1100\_1200\_0.5\_2000 & 149402          & 148618.4 &  & \textbf{150118}   & 149543.9 \\
bmcp\_1200\_1100\_0.3\_3000 & \textbf{161848} & 159267.2 &  & \textbf{161848}   & 161677.3 \\
bmcp\_1200\_1100\_0.5\_2000 & 136073          & 135347.1 &  & \textbf{137166}   & 136345.6 \\
bmcp\_1200\_1200\_0.3\_3000 & 169219          & 168710.1 &  & \textbf{172163}   & 171676.4 \\
bmcp\_1200\_1200\_0.5\_2000 & 148706          & 147717.1 &  & \textbf{149654}   & 148778.7 \\
bmcp\_1200\_1300\_0.3\_3000 & 184156          & 181891.2 &  & \textbf{184219}   & 183521.0 \\
bmcp\_1200\_1300\_0.5\_2000 & 160487          & 159181.1 &  & \textbf{161499}   & 160696.5 \\
bmcp\_1300\_1200\_0.3\_3000 & 168304          & 167883.9 &  & \textbf{170283}   & 169472.6 \\
bmcp\_1300\_1200\_0.5\_2000 & 150249          & 148937.0 &  & \textbf{151402}   & 150644.3 \\
bmcp\_1300\_1300\_0.3\_3000 & 180593          & 179909.5 &  & \textbf{184429}   & 183001.0 \\
bmcp\_1300\_1300\_0.5\_2000 & 160677          & 159351.7 &  & \textbf{161652}   & 161140.9 \\
bmcp\_1300\_1400\_0.3\_3000 & 195341          & 195308.4 &  & \textbf{199134}   & 198425.0 \\
bmcp\_1300\_1400\_0.5\_2000 & 172244          & 171175.5 &  & \textbf{173954}   & 173383.3 \\
bmcp\_1400\_1300\_0.3\_3000 & 181154          & 179794.4 &  & \textbf{183987}   & 183365.9 \\
bmcp\_1400\_1300\_0.5\_2000 & 161658          & 159182.6 &  & \textbf{162506}   & 161797.7 \\
bmcp\_1400\_1400\_0.3\_3000 & 199067          & 197227.7 &  & \textbf{199973}   & 199312.9 \\
bmcp\_1400\_1400\_0.5\_2000 & 173693          & 172899.6 &  & \textbf{174912}   & 173614.3 \\
bmcp\_1400\_1500\_0.3\_3000 & 210450          & 208051.0 &  & \textbf{212492}   & 210916.3 \\
bmcp\_1400\_1500\_0.5\_2000 & 183146          & 182427.8 &  & \textbf{186036}   & 185586.7 \\
bmcp\_1500\_1400\_0.3\_3000 & 193676          & 192820.3 &  & \textbf{197184}   & 196418.0 \\
bmcp\_1500\_1400\_0.5\_2000 & 171949          & 170581.2 &  & \textbf{174216}   & 173276.0 \\
bmcp\_1500\_1500\_0.3\_3000 & 208630          & 206404.9 &  & \textbf{211108}   & 210037.7 \\
bmcp\_1500\_1500\_0.5\_2000 & 183599          & 181456.4 &  & \textbf{186311}   & 184810.1 \\
bmcp\_1500\_1600\_0.3\_3000 & \textbf{226408} & 221501.2 &  & 225279            & 224205.2 \\
bmcp\_1500\_1600\_0.5\_2000 & 197566          & 195828.2 &  & \textbf{198069}   & 197614.9 \\ \hline
Average                     & 171984.2        & 170631.9 &  & \textbf{173642.1} & 172842.6 \\ \hline
\multicolumn{6}{l}{30 minutes of time limit}                                               \\ \hline
bmcp\_1100\_1000\_0.3\_3000 & 142835          & 142428.7 &  & \textbf{143402}   & 143160.2 \\
bmcp\_1100\_1000\_0.5\_2000 & 125974          & 125790.0 &  & \textbf{127157}   & 126253.1 \\
bmcp\_1100\_1100\_0.3\_3000 & 154936          & 154661.7 &  & \textbf{157530}   & 156962.4 \\
bmcp\_1100\_1100\_0.5\_2000 & \textbf{139196} & 138169.0 &  & \textbf{139196}   & 138716.5 \\
bmcp\_1100\_1200\_0.3\_3000 & 169113          & 168763.6 &  & \textbf{172660}   & 172114.0 \\
bmcp\_1100\_1200\_0.5\_2000 & 150301          & 149366.4 &  & \textbf{150493}   & 150043.9 \\
bmcp\_1200\_1100\_0.3\_3000 & \textbf{161848} & 159620.3 &  & \textbf{161848}   & 161848.0 \\
bmcp\_1200\_1100\_0.5\_2000 & 135858          & 135509.2 &  & \textbf{137700}   & 136765.6 \\
bmcp\_1200\_1200\_0.3\_3000 & 169219          & 168821.7 &  & \textbf{172595}   & 172081.1 \\
bmcp\_1200\_1200\_0.5\_2000 & 149654 & 148679.1  &  & \textbf{149902}            & 149334.4 \\
bmcp\_1200\_1300\_0.3\_3000 & 183004          & 182220.4 &  & \textbf{184431}   & 183686.8 \\
bmcp\_1200\_1300\_0.5\_2000 & 160369          & 159735.4 &  & \textbf{161662}   & 161074.5 \\
bmcp\_1300\_1200\_0.3\_3000 & 168586          & 168473.8 &  & \textbf{170283}   & 169800.5 \\
bmcp\_1300\_1200\_0.5\_2000 & 151067          & 150034.7 &  & \textbf{151512}   & 151053.2 \\
bmcp\_1300\_1300\_0.3\_3000 & 180608          & 179978.4 &  & \textbf{184699}   & 183427.8 \\
bmcp\_1300\_1300\_0.5\_2000 & 160485          & 159511.3 &  & \textbf{162146}   & 161523.8 \\
bmcp\_1300\_1400\_0.3\_3000 & 197709          & 195681.9 &  & \textbf{199134}   & 198913.4 \\
bmcp\_1300\_1400\_0.5\_2000 & 173349          & 171665.0 &  & \textbf{173954}   & 173773.5 \\
bmcp\_1400\_1300\_0.3\_3000 & 182881          & 180143.5 &  & \textbf{184148}   & 183536.2 \\
bmcp\_1400\_1300\_0.5\_2000 & 161995          & 160647.0 &  & \textbf{162544}   & 162324.7 \\
bmcp\_1400\_1400\_0.3\_3000 & 199879          & 197229.0 &  & \textbf{200136}   & 199714.5 \\
bmcp\_1400\_1400\_0.5\_2000 & 174683          & 173393.1 &  & \textbf{175583}   & 174370.2 \\
bmcp\_1400\_1500\_0.3\_3000 & 210077          & 208315.6 &  & \textbf{212492}   & 211356.6 \\
bmcp\_1400\_1500\_0.5\_2000 & 184259          & 183289.9 &  & \textbf{186818}   & 185991.7 \\
bmcp\_1500\_1400\_0.3\_3000 & 194156          & 193554.8 &  & \textbf{197899}   & 196753.8 \\
bmcp\_1500\_1400\_0.5\_2000 & 173475          & 171426.9 &  & \textbf{174522}   & 173745.1 \\
bmcp\_1500\_1500\_0.3\_3000 & 209929          & 207795.3 &  & \textbf{211108}   & 210451.1 \\
bmcp\_1500\_1500\_0.5\_2000 & 184082          & 182676.2 &  & \textbf{187052}   & 185464.7 \\
bmcp\_1500\_1600\_0.3\_3000 & \textbf{226408} & 221641.3 &  & \textbf{226408}   & 225031.9 \\
bmcp\_1500\_1600\_0.5\_2000 & 198214          & 196659.0 &  & \textbf{198579}   & 198258.0 \\ \hline
Average                     & 172471.6         & 171196.1  &  & \textbf{173919.8} & 173251.0 \\ \bottomrule
\end{tabular}}
\end{table}

==> table3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[b]
\centering
\caption{Comparison results of VDLS and PLTS, with 10 or 30 minutes of time limit, on the 30 instances of the third set. Best results appear in bold.}
\label{table3}
\scalebox{0.65}{\begin{tabular}{lrrrrr} \toprule
\multirow{2}{*}{Instances}   & \multicolumn{2}{r}{PLTS} &  & \multicolumn{2}{r}{VDLS}       \\ \cline{2-3} \cline{5-6} 
                             & best        & average    &  & best               & average   \\ \hline
\multicolumn{6}{l}{10 minutes of time limit}                                                \\ \hline
bmcp\_4200\_4000\_0.3\_10000 & 1775432     & 1736438.9  &  & \textbf{1830682}   & 1822544.7 \\
bmcp\_4200\_4000\_0.5\_7000  & 1692056     & 1662063.5  &  & \textbf{1723412}   & 1714352.7 \\
bmcp\_4200\_4200\_0.3\_10000 & 1856948     & 1824810.6  &  & \textbf{1916508}   & 1910284.8 \\
bmcp\_4200\_4200\_0.5\_7000  & 1759417     & 1735178.9  &  & \textbf{1801380}   & 1794520.8 \\
bmcp\_4200\_4400\_0.3\_10000 & 1964294     & 1928237.3  &  & \textbf{2018747}   & 2010704.6 \\
bmcp\_4200\_4400\_0.5\_7000  & 1846157     & 1815658.3  &  & \textbf{1892758}   & 1878894.0 \\
bmcp\_4400\_4200\_0.3\_10000 & 1817604     & 1797114.8  &  & \textbf{1906626}   & 1901442.2 \\
bmcp\_4400\_4200\_0.5\_7000  & 1762870     & 1724377.3  &  & \textbf{1803620}   & 1795038.9 \\
bmcp\_4400\_4400\_0.3\_10000 & 1948267     & 1918148.4  &  & \textbf{2019258}   & 2011327.9 \\
bmcp\_4400\_4400\_0.5\_7000  & 1817416     & 1806039.0  &  & \textbf{1881802}   & 1870369.4 \\
bmcp\_4400\_4600\_0.3\_10000 & 2016242     & 1989001.0  &  & \textbf{2088441}   & 2082175.3 \\
bmcp\_4400\_4600\_0.5\_7000  & 1913938     & 1895993.0  &  & \textbf{1975347}   & 1969960.7 \\
bmcp\_4600\_4400\_0.3\_10000 & 1939966     & 1894543.2  &  & \textbf{2001130}   & 1990786.6 \\
bmcp\_4600\_4400\_0.5\_7000  & 1822083     & 1803727.3  &  & \textbf{1887466}   & 1883406.3 \\
bmcp\_4600\_4600\_0.3\_10000 & 2027745     & 1996365.4  &  & \textbf{2094216}   & 2083473.6 \\
bmcp\_4600\_4600\_0.5\_7000  & 1932145     & 1886756.8  &  & \textbf{1971725}   & 1964079.9 \\
bmcp\_4600\_4800\_0.3\_10000 & 2090814     & 2062236.5  &  & \textbf{2190154}   & 2185272.7 \\
bmcp\_4600\_4800\_0.5\_7000  & 2006997     & 1964777.6  &  & \textbf{2057735}   & 2046486.2 \\
bmcp\_4800\_4600\_0.3\_10000 & 2008566     & 1974395.8  &  & \textbf{2083384}   & 2071702.3 \\
bmcp\_4800\_4600\_0.5\_7000  & 1902428     & 1879771.0  &  & \textbf{1971497}   & 1961059.4 \\
bmcp\_4800\_4800\_0.3\_10000 & 2071733     & 2034925.5  &  & \textbf{2174319}   & 2161654.4 \\
bmcp\_4800\_4800\_0.5\_7000  & 1981902     & 1955184.4  &  & \textbf{2056296}   & 2045562.0 \\
bmcp\_4800\_5000\_0.3\_10000 & 2221536     & 2157486.8  &  & \textbf{2269467}   & 2264154.8 \\
bmcp\_4800\_5000\_0.5\_7000  & 2055213     & 2032723.9  &  & \textbf{2128014}   & 2123405.0 \\
bmcp\_5000\_4800\_0.3\_10000 & 2076374     & 2039438.7  &  & \textbf{2170753}   & 2160307.7 \\
bmcp\_5000\_4800\_0.5\_7000  & 1987069     & 1962373.3  &  & \textbf{2051568}   & 2045975.6 \\
bmcp\_5000\_5000\_0.3\_10000 & 2154362     & 2103199.9  &  & \textbf{2251341}   & 2237813.2 \\
bmcp\_5000\_5000\_0.5\_7000  & 2077170     & 2041834.9  &  & \textbf{2145927}   & 2132536.3 \\
bmcp\_5000\_5200\_0.3\_10000 & 2235890     & 2211542.6  &  & \textbf{2342235}   & 2334076.7 \\
bmcp\_5000\_5200\_0.5\_7000  & 2119204     & 2099244.2  &  & \textbf{2209415}   & 2197764.2 \\ \hline
Average                      & 1962727.9   & 1931119.6  &  & \textbf{2030507.4} & 2021704.4 \\ \hline
\multicolumn{6}{l}{30 minutes of time limit}                                                \\ \hline
bmcp\_4200\_4000\_0.3\_10000 & 1778013     & 1747411.9  &  & \textbf{1835947}   & 1828442.4 \\
bmcp\_4200\_4000\_0.5\_7000  & 1685141     & 1666673.3  &  & \textbf{1733033}   & 1724198.8 \\
bmcp\_4200\_4200\_0.3\_10000 & 1874190     & 1839780.1  &  & \textbf{1922985}   & 1915332.4 \\
bmcp\_4200\_4200\_0.5\_7000  & 1764277     & 1742121.7  &  & \textbf{1802880}   & 1798430.9 \\
bmcp\_4200\_4400\_0.3\_10000 & 1954069     & 1932251.0  &  & \textbf{2022834}   & 2016260.1 \\
bmcp\_4200\_4400\_0.5\_7000  & 1853677     & 1820444.4  &  & \textbf{1894307}   & 1883721.0 \\
bmcp\_4400\_4200\_0.3\_10000 & 1833465     & 1816879.1  &  & \textbf{1911617}   & 1905971.7 \\
bmcp\_4400\_4200\_0.5\_7000  & 1746064     & 1730783.9  &  & \textbf{1807860}   & 1799645.5 \\
bmcp\_4400\_4400\_0.3\_10000 & 1945218     & 1922134.2  &  & \textbf{2023432}   & 2019636.3 \\
bmcp\_4400\_4400\_0.5\_7000  & 1844031     & 1821467.8  &  & \textbf{1888693}   & 1882463.1 \\
bmcp\_4400\_4600\_0.3\_10000 & 2003959     & 1993946.2  &  & \textbf{2097123}   & 2088349.1 \\
bmcp\_4400\_4600\_0.5\_7000  & 1937066     & 1906956.1  &  & \textbf{1981337}   & 1973941.3 \\
bmcp\_4600\_4400\_0.3\_10000 & 1930498     & 1913501.0  &  & \textbf{2011730}   & 1998707.0 \\
bmcp\_4600\_4400\_0.5\_7000  & 1845046     & 1817697.2  &  & \textbf{1897119}   & 1889599.7 \\
bmcp\_4600\_4600\_0.3\_10000 & 2027132     & 2005096.7  &  & \textbf{2103476}   & 2093832.3 \\
bmcp\_4600\_4600\_0.5\_7000  & 1921261     & 1900376.3  &  & \textbf{1976832}   & 1970554.1 \\
bmcp\_4600\_4800\_0.3\_10000 & 2120120     & 2091722.5  &  & \textbf{2200580}   & 2193619.0 \\
bmcp\_4600\_4800\_0.5\_7000  & 1989454     & 1967943.3  &  & \textbf{2064098}   & 2053550.3 \\
bmcp\_4800\_4600\_0.3\_10000 & 2019033     & 1991673.5  &  & \textbf{2093497}   & 2081197.6 \\
bmcp\_4800\_4600\_0.5\_7000  & 1922466     & 1901157.6  &  & \textbf{1977557}   & 1969484.1 \\
bmcp\_4800\_4800\_0.3\_10000 & 2100773     & 2058921.6  &  & \textbf{2180165}   & 2171120.6 \\
bmcp\_4800\_4800\_0.5\_7000  & 2009129     & 1973993.6  &  & \textbf{2058797}   & 2053170.9 \\
bmcp\_4800\_5000\_0.3\_10000 & 2184445     & 2157793.0  &  & \textbf{2275455}   & 2270224.7 \\
bmcp\_4800\_5000\_0.5\_7000  & 2087596     & 2050741.0  &  & \textbf{2133843}   & 2129594.0 \\
bmcp\_5000\_4800\_0.3\_10000 & 2069979     & 2051607.2  &  & \textbf{2181584}   & 2167254.8 \\
bmcp\_5000\_4800\_0.5\_7000  & 2013921     & 1977310.7  &  & \textbf{2061909}   & 2053025.7 \\
bmcp\_5000\_5000\_0.3\_10000 & 2144223     & 2126462.9  &  & \textbf{2254007}   & 2247746.1 \\
bmcp\_5000\_5000\_0.5\_7000  & 2067188     & 2046886.5  &  & \textbf{2145927}   & 2135823.3 \\
bmcp\_5000\_5200\_0.3\_10000 & 2231359     & 2220887.2  &  & \textbf{2352676}   & 2340288.0 \\
bmcp\_5000\_5200\_0.5\_7000  & 2129556     & 2115338.3  &  & \textbf{2224001}   & 2207572.4 \\ \hline
Average                      & 1967745.0   & 1943665.3  &  & \textbf{2037176.7} & 2028758.6 \\ \bottomrule
\end{tabular}}
\end{table}

==> table_v1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\caption{Comparison of the VDLS and its variant algorithms, VDLS$_{full}$ and VDLS$_{random}$, with 30 minutes of time limit in solving the 30 instances of the first set. Best results appear in bold.}
\label{table_v1}
\scalebox{0.65}{\begin{tabular}{lrrrrrrrr} \toprule
\multirow{2}{*}{Instances}    & \multicolumn{2}{r}{VDLS$_{full}$} &  & \multicolumn{2}{r}{VDLS$_{random}$} &  & \multicolumn{2}{r}{VDLS}    \\ \cline{2-3} \cline{5-6} \cline{8-9} 
                              & best                & average     &  & best                & average       &  & best             & average  \\ \hline
bmcp\_585\_600\_0.05\_2000    & \textbf{71091}      & 71027.1     &  & 70752               & 70560.5       &  & \textbf{71091}   & 71006.5  \\
bmcp\_585\_600\_0.075\_1500   & \textbf{71025}      & 70666.2     &  & 70545               & 70119.7       &  & \textbf{71025}   & 70554.2  \\
bmcp\_600\_585\_0.05\_2000    & \textbf{67636}      & 67583.1     &  & 67482               & 67373.6       &  & \textbf{67636}   & 67621.6  \\
bmcp\_600\_585\_0.075\_1500   & 70362               & 70243.2     &  & 70099               & 69678.9       &  & \textbf{70588}   & 70367.1  \\
bmcp\_600\_600\_0.05\_2000    & \textbf{68738}      & 68497.5     &  & 67912               & 67688.5       &  & \textbf{68738}   & 68559.9  \\
bmcp\_600\_600\_0.075\_1500   & \textbf{71904}      & 71815.5     &  & \textbf{71904}      & 71592.7       &  & \textbf{71904}   & 71833.2  \\
bmcp\_685\_700\_0.05\_2000    & \textbf{80751}      & 80304.6     &  & 80121               & 79835.1       &  & \textbf{80751}   & 80388.7  \\
bmcp\_685\_700\_0.075\_1500   & 82955               & 82683.4     &  & 82456               & 82020.7       &  & \textbf{83286}   & 82870.3  \\
bmcp\_700\_685\_0.05\_2000    & \textbf{78054}      & 77738.4     &  & 77039               & 76859.7       &  & \textbf{78054}   & 77674.4  \\
bmcp\_700\_685\_0.075\_1500   & \textbf{78869}      & 78573.7     &  & 78395               & 77276.3       &  & \textbf{78869}   & 78649.1  \\
bmcp\_700\_700\_0.05\_2000    & \textbf{78458}      & 78105.8     &  & 77512               & 77090.4       &  & \textbf{78458}   & 78252.7  \\
bmcp\_700\_700\_0.075\_1500   & \textbf{84576}      & 84576.0     &  & 84229               & 83613.7       &  & \textbf{84576}   & 84576.0  \\
bmcp\_785\_800\_0.05\_2000    & 92454               & 92218.1     &  & 92057               & 91377.8       &  & \textbf{92630}   & 92400.1  \\
bmcp\_785\_800\_0.075\_1500   & \textbf{95221}      & 95221.0     &  & 94889               & 94826.8       &  & \textbf{95221}   & 95221.0  \\
bmcp\_800\_785\_0.05\_2000    & \textbf{89138}      & 88834.7     &  & 89007               & 88013.8       &  & \textbf{89138}   & 89024.7  \\
bmcp\_800\_785\_0.075\_1500   & \textbf{91856}      & 91674.0     &  & 91271               & 90859.4       &  & \textbf{91856}   & 91644.6  \\
bmcp\_800\_800\_0.05\_2000    & 91711               & 91614.9     &  & 90295               & 90083.0       &  & \textbf{91795}   & 91541.8  \\
bmcp\_800\_800\_0.075\_1500   & \textbf{95995}      & 95504.7     &  & 95168               & 94512.0       &  & \textbf{95995}   & 95652.6  \\
bmcp\_885\_900\_0.05\_2000    & \textbf{102277}     & 102040.3    &  & 100908              & 100313.6      &  & \textbf{102277}  & 101853.2 \\
bmcp\_885\_900\_0.075\_1500   & \textbf{106940}     & 106598.4    &  & 106120              & 105856.1      &  & \textbf{106940}  & 106477.2 \\
bmcp\_900\_885\_0.05\_2000    & \textbf{99590}      & 99192.5     &  & 98841               & 98496.2       &  & \textbf{99590}   & 99289.1  \\
bmcp\_900\_885\_0.075\_1500   & \textbf{105141}     & 105091.2    &  & 104826              & 103715.0      &  & \textbf{105141}  & 104991.6 \\
bmcp\_900\_900\_0.05\_2000    & 101226              & 100935.2    &  & 99806               & 99222.9       &  & \textbf{101857}  & 101089.2 \\
bmcp\_900\_900\_0.075\_1500   & \textbf{105081}     & 104915.1    &  & 103838              & 103804.2      &  & \textbf{105081}  & 104955.7 \\
bmcp\_985\_1000\_0.05\_2000   & \textbf{110669}     & 109524.6    &  & 108605              & 108250.3      &  & 110319           & 109673.1 \\
bmcp\_985\_1000\_0.075\_1500  & 115348              & 114813.8    &  & 113789              & 113391.3      &  & \textbf{115505}  & 115075.4 \\
bmcp\_1000\_1000\_0.05\_2000  & \textbf{113331}     & 113076.3    &  & 112826              & 111996.4      &  & \textbf{113331}  & 113096.6 \\
bmcp\_1000\_1000\_0.075\_1500 & \textbf{120246}     & 119922.0    &  & 119301              & 118937.4      &  & \textbf{120246}  & 119939.3 \\
bmcp\_1000\_985\_0.05\_2000   & \textbf{112057}     & 111567.7    &  & 111328              & 109475.4      &  & \textbf{112057}  & 111552.3 \\
bmcp\_1000\_985\_0.075\_1500  & 113029              & 112722.3    &  & 112858              & 111960.8      &  & \textbf{113615}  & 112984.4 \\ \hline
Average                       & 92191.0             & 91909.4     &  & 91472.6             & 90960.1       &  & \textbf{92252.3} & 91960.5 \\ \bottomrule
\end{tabular}}
\end{table}

==> table_v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\caption{Comparison of the VDLS and its variant algorithms, VDLS$_{full}$ and VDLS$_{random}$, with 30 minutes of time limit in solving the 30 instances of the second set. Best results appear in bold.}
\label{table_v2}
\scalebox{0.6}{\begin{tabular}{lrrrrrrrr} \toprule
\multirow{2}{*}{Instances}  & \multicolumn{2}{r}{VDLS$_{full}$} &  & \multicolumn{2}{r}{VDLS$_{random}$} &  & \multicolumn{2}{r}{VDLS}     \\ \cline{2-3} \cline{5-6} \cline{8-9} 
                            & best                & average     &  & best             & average          &  & best              & average  \\ \hline
bmcp\_1100\_1000\_0.3\_3000 & \textbf{143402}     & 142860.1    &  & 141054           & 141054.0         &  & \textbf{143402}   & 142990.1 \\
bmcp\_1100\_1000\_0.5\_2000 & 126873              & 125965.5    &  & 125223           & 125223.0         &  & \textbf{126935}   & 126022.2 \\
bmcp\_1100\_1100\_0.3\_3000 & \textbf{157530}     & 156269.3    &  & 155671           & 155669.2         &  & \textbf{157530}   & 156888.7 \\
bmcp\_1100\_1100\_0.5\_2000 & \textbf{139141}     & 138594.2    &  & 135069           & 134757.6         &  & \textbf{139141}   & 138565.5 \\
bmcp\_1100\_1200\_0.3\_3000 & \textbf{172660}     & 171548.9    &  & 170088           & 169023.3         &  & \textbf{172660}   & 171548.7 \\
bmcp\_1100\_1200\_0.5\_2000 & \textbf{150197}     & 149190.2    &  & 146698           & 146249.3         &  & 150118            & 149543.9 \\
bmcp\_1200\_1100\_0.3\_3000 & \textbf{161848}     & 161627.7    &  & 160518           & 160107.2         &  & \textbf{161848}   & 161677.3 \\
bmcp\_1200\_1100\_0.5\_2000 & 136832              & 136297.9    &  & 134575           & 134272.2         &  & \textbf{137166}   & 136345.6 \\
bmcp\_1200\_1200\_0.3\_3000 & \textbf{172595}     & 171410.7    &  & 169196           & 168489.9         &  & 172163            & 171676.4 \\
bmcp\_1200\_1200\_0.5\_2000 & 149137              & 148742.2    &  & 147670           & 146861.1         &  & \textbf{149654}   & 148778.7 \\
bmcp\_1200\_1300\_0.3\_3000 & 183634              & 183046.7    &  & 181849           & 180940.0         &  & \textbf{184219}   & 183521.0 \\
bmcp\_1200\_1300\_0.5\_2000 & \textbf{162029}     & 160738.4    &  & 158385           & 156583.5         &  & 161499            & 160696.5 \\
bmcp\_1300\_1200\_0.3\_3000 & \textbf{170372}     & 169556.9    &  & 167566           & 166955.2         &  & 170283            & 169472.6 \\
bmcp\_1300\_1200\_0.5\_2000 & 150726              & 150200.3    &  & 148732           & 147361.7         &  & \textbf{151402}   & 150644.3 \\
bmcp\_1300\_1300\_0.3\_3000 & \textbf{184618}     & 182641.7    &  & 181474           & 180229.4         &  & 184429            & 183001.0 \\
bmcp\_1300\_1300\_0.5\_2000 & \textbf{162032}     & 161025.8    &  & 159170           & 158281.3         &  & 161652            & 161140.9 \\
bmcp\_1300\_1400\_0.3\_3000 & 199058              & 198401.2    &  & 194989           & 193512.0         &  & \textbf{199134}   & 198425.0 \\
bmcp\_1300\_1400\_0.5\_2000 & 173891              & 173170.6    &  & 171385           & 170938.5         &  & \textbf{173954}   & 173383.3 \\
bmcp\_1400\_1300\_0.3\_3000 & 183537              & 182925.1    &  & 181595           & 179861.1         &  & \textbf{183987}   & 183365.9 \\
bmcp\_1400\_1300\_0.5\_2000 & 162082              & 161630.5    &  & 160692           & 160109.4         &  & \textbf{162506}   & 161797.7 \\
bmcp\_1400\_1400\_0.3\_3000 & 199607              & 198747.1    &  & 197449           & 194877.1         &  & \textbf{199973}   & 199312.9 \\
bmcp\_1400\_1400\_0.5\_2000 & 173864              & 173483.7    &  & 170964           & 169975.6         &  & \textbf{174912}   & 173614.3 \\
bmcp\_1400\_1500\_0.3\_3000 & 212115              & 210705.6    &  & 208432           & 207656.3         &  & \textbf{212492}   & 210916.3 \\
bmcp\_1400\_1500\_0.5\_2000 & \textbf{186061}     & 185722.9    &  & 184174           & 183537.4         &  & 186036            & 185586.7 \\
bmcp\_1500\_1400\_0.3\_3000 & \textbf{197184}     & 196459.2    &  & 194100           & 192343.3         &  & \textbf{197184}   & 196418.0 \\
bmcp\_1500\_1400\_0.5\_2000 & \textbf{174216}     & 173087.1    &  & 171257           & 170973.2         &  & \textbf{174216}   & 173276.0 \\
bmcp\_1500\_1500\_0.3\_3000 & 210117              & 209517.0    &  & 207670           & 206587.9         &  & \textbf{211108}   & 210037.7 \\
bmcp\_1500\_1500\_0.5\_2000 & 185900              & 184789.0    &  & 184010           & 182099.5         &  & \textbf{186311}   & 184810.1 \\
bmcp\_1500\_1600\_0.3\_3000 & \textbf{225358}     & 223179.2    &  & 221358           & 220159.2         &  & 225279            & 224205.2 \\
bmcp\_1500\_1600\_0.5\_2000 & \textbf{198148}     & 197705.4    &  & 196616           & 196221.8         &  & 198069            & 197614.9 \\ \hline
Average                     & 173492.1            & 172641.3    &  & 170921.0         & 170030.3         &  & \textbf{173642.1} & 172842.6 \\ \bottomrule \vspace{-2em}
\end{tabular}}
\end{table}

==> table_v3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[b]
\centering
\caption{Comparison of the VDLS and its variant algorithms, VDLS$_{full}$ and VDLS$_{random}$, with 30 minutes of time limit in solving the 30 instances of the third set. Best results appear in bold.}
\label{table_v3}
\scalebox{0.56}{\begin{tabular}{lrrrrrrrr} \toprule
\multirow{2}{*}{Instances}   & \multicolumn{2}{r}{VDLS$_{full}$} &  & \multicolumn{2}{r}{VDLS$_{random}$} &  & \multicolumn{2}{r}{VDLS}       \\ \cline{2-3} \cline{5-6} \cline{8-9} 
                             & best                & average     &  & best             & average          &  & best               & average   \\ \hline
bmcp\_4200\_4000\_0.3\_10000 & \textbf{1834932}    & 1819901.5   &  & 1789126          & 1787440.4        &  & 1830682            & 1822544.7 \\
bmcp\_4200\_4000\_0.5\_7000  & 1719732             & 1713648.7   &  & 1696280          & 1696280.0        &  & \textbf{1723412}   & 1714352.7 \\
bmcp\_4200\_4200\_0.3\_10000 & 1913286             & 1906685.4   &  & 1890316          & 1890316.0        &  & \textbf{1916508}   & 1910284.8 \\
bmcp\_4200\_4200\_0.5\_7000  & \textbf{1804255}    & 1795403.0   &  & 1778044          & 1776970.3        &  & 1801380            & 1794520.8 \\
bmcp\_4200\_4400\_0.3\_10000 & 2013804             & 2008907.7   &  & 1999738          & 1996957.9        &  & \textbf{2018747}   & 2010704.6 \\
bmcp\_4200\_4400\_0.5\_7000  & 1885015             & 1876342.6   &  & 1863931          & 1862810.5        &  & \textbf{1892758}   & 1878894.0 \\
bmcp\_4400\_4200\_0.3\_10000 & 1905269             & 1898725.5   &  & 1884808          & 1884808.0        &  & \textbf{1906626}   & 1901442.2 \\
bmcp\_4400\_4200\_0.5\_7000  & 1800778             & 1795823.9   &  & 1787968          & 1787968.0        &  & \textbf{1803620}   & 1795038.9 \\
bmcp\_4400\_4400\_0.3\_10000 & \textbf{2024016}    & 2011642.7   &  & 1997381          & 1997381.0        &  & 2019258            & 2011327.9 \\
bmcp\_4400\_4400\_0.5\_7000  & \textbf{1883483}    & 1871501.5   &  & 1847671          & 1846956.4        &  & 1881802            & 1870369.4 \\
bmcp\_4400\_4600\_0.3\_10000 & \textbf{2091966}    & 2078506.8   &  & 2067837          & 2066053.2        &  & 2088441            & 2082175.3 \\
bmcp\_4400\_4600\_0.5\_7000  & \textbf{1979369}    & 1971599.0   &  & 1966265          & 1966265.0        &  & 1975347            & 1969960.7 \\
bmcp\_4600\_4400\_0.3\_10000 & 1995199             & 1989104.0   &  & 1968554          & 1968554.0        &  & \textbf{2001130}   & 1990786.6 \\
bmcp\_4600\_4400\_0.5\_7000  & \textbf{1890025}    & 1883976.7   &  & 1880145          & 1880145.0        &  & 1887466            & 1883406.3 \\
bmcp\_4600\_4600\_0.3\_10000 & \textbf{2095805}    & 2085495.3   &  & 2066933          & 2062183.7        &  & 2094216            & 2083473.6 \\
bmcp\_4600\_4600\_0.5\_7000  & \textbf{1973758}    & 1965042.8   &  & 1953192          & 1953192.0        &  & 1971725            & 1964079.9 \\
bmcp\_4600\_4800\_0.3\_10000 & \textbf{2191427}    & 2181604.2   &  & 2174210          & 2171744.0        &  & 2190154            & 2185272.7 \\
bmcp\_4600\_4800\_0.5\_7000  & \textbf{2058129}    & 2047568.8   &  & 2038326          & 2036013.0        &  & 2057735            & 2046486.2 \\
bmcp\_4800\_4600\_0.3\_10000 & 2082765             & 2072201.4   &  & 2055216          & 2055216.0        &  & \textbf{2083384}   & 2071702.3 \\
bmcp\_4800\_4600\_0.5\_7000  & 1967434             & 1961564.0   &  & 1939019          & 1937578.3        &  & \textbf{1971497}   & 1961059.4 \\
bmcp\_4800\_4800\_0.3\_10000 & 2172841             & 2161567.8   &  & 2142300          & 2142300.0        &  & \textbf{2174319}   & 2161654.4 \\
bmcp\_4800\_4800\_0.5\_7000  & 2056211             & 2046674.5   &  & 2031280          & 2029781.8        &  & \textbf{2056296}   & 2045562.0 \\
bmcp\_4800\_5000\_0.3\_10000 & \textbf{2270783}    & 2267523.2   &  & 2261424          & 2261424.0        &  & 2269467            & 2264154.8 \\
bmcp\_4800\_5000\_0.5\_7000  & \textbf{2128223}    & 2122463.9   &  & 2110025          & 2110025.0        &  & 2128014            & 2123405.0 \\
bmcp\_5000\_4800\_0.3\_10000 & \textbf{2173965}    & 2157271.1   &  & 2132141          & 2130486.8        &  & 2170753            & 2160307.7 \\
bmcp\_5000\_4800\_0.5\_7000  & 2050437             & 2045379.8   &  & 2036595          & 2036595.0        &  & \textbf{2051568}   & 2045975.6 \\
bmcp\_5000\_5000\_0.3\_10000 & 2250550             & 2240244.3   &  & 2221594          & 2221594.0        &  & \textbf{2251341}   & 2237813.2 \\
bmcp\_5000\_5000\_0.5\_7000  & 2140256             & 2132516.5   &  & 2119843          & 2119843.0        &  & \textbf{2145927}   & 2132536.3 \\
bmcp\_5000\_5200\_0.3\_10000 & 2339720             & 2327075.1   &  & 2313915          & 2310933.3        &  & \textbf{2342235}   & 2334076.7 \\
bmcp\_5000\_5200\_0.5\_7000  & \textbf{2214316}    & 2201192.0   &  & 2196497          & 2191668.5        &  & 2209415            & 2197764.2 \\ \hline
Average                      & 2030258.3           & 2021238.5   &  & 2007019.1        & 2005982.8        &  & \textbf{2030507.4} & 2021704.4 \\ \bottomrule \vspace{-2.5em}
\end{tabular}}
\end{table}

==> table_v4.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[b]
\centering
\caption{Comparison of the VDLS and its variant algorithms, VDLS$_{empty\_init}$ and VDLS$_{random\_init}$, as well as the PLTS algorithm, with 30 minutes of time limit in solving the 30 instances of the first set. Best results appear in bold.}
\label{table_v4}
\scalebox{0.6}{\begin{tabular}{lrrrrrrrrrrr} \toprule
\multirow{2}{*}{Instances}    & \multicolumn{2}{r}{PLTS}   &  & \multicolumn{2}{r}{VDLS$_{empty\_init}$} &  & \multicolumn{2}{r}{VDLS$_{random\_init}$} &  & \multicolumn{2}{r}{VDLS}    \\ \cline{2-3} \cline{5-6} \cline{8-9} \cline{11-12} 
                              & best            & average  &  & best                   & average         &  & best                    & average         &  & best             & average  \\ \hline
bmcp\_585\_600\_0.05\_2000    & \textbf{71102}  & 70915.0  &  & \textbf{71102}         & 71026.1         &  & \textbf{71102}          & 70981.7         &  & 71091            & 71025.0  \\
bmcp\_585\_600\_0.075\_1500   & 70677           & 70670.2  &  & \textbf{71025}         & 70656.8         &  & \textbf{71025}          & 70689.7         &  & \textbf{71025}   & 70554.2  \\
bmcp\_600\_585\_0.05\_2000    & \textbf{67636}  & 67041.5  &  & \textbf{67636}         & 67437.9         &  & \textbf{67636}          & 67560.0         &  & \textbf{67636}   & 67621.6  \\
bmcp\_600\_585\_0.075\_1500   & 70318           & 70318.0  &  & \textbf{70588}         & 70310.3         &  & \textbf{70588}          & 70241.5         &  & \textbf{70588}   & 70371.7  \\
bmcp\_600\_600\_0.05\_2000    & 68453           & 68386.8  &  & \textbf{68738}         & 68541.1         &  & \textbf{68738}          & 68577.4         &  & \textbf{68738}   & 68620.1  \\
bmcp\_600\_600\_0.075\_1500   & 71746           & 71746.0  &  & \textbf{71904}         & 71724.6         &  & \textbf{71904}          & 71764.3         &  & \textbf{71904}   & 71833.2  \\
bmcp\_685\_700\_0.05\_2000    & 80197           & 80096.6  &  & \textbf{81227}         & 80939.4         &  & \textbf{81227}          & 80901.3         &  & \textbf{81227}   & 80551.6  \\
bmcp\_685\_700\_0.075\_1500   & 82955           & 82944.2  &  & \textbf{83286}         & 82765.4         &  & 82955                   & 82822.7         &  & \textbf{83286}   & 82870.3  \\
bmcp\_700\_685\_0.05\_2000    & 77876           & 77372.7  &  & \textbf{78054}         & 77804.5         &  & \textbf{78054}          & 77734.9         &  & \textbf{78054}   & 77780.5  \\
bmcp\_700\_685\_0.075\_1500   & \textbf{78869}  & 78810.4  &  & \textbf{78869}         & 78712.6         &  & \textbf{78869}          & 78757.0         &  & \textbf{78869}   & 78649.1  \\
bmcp\_700\_700\_0.05\_2000    & 78028           & 77501.5  &  & \textbf{78458}         & 78113.0         &  & \textbf{78458}          & 78128.1         &  & \textbf{78458}   & 78304.8  \\
bmcp\_700\_700\_0.075\_1500   & 84570           & 83720.7  &  & \textbf{84576}         & 84576.0         &  & \textbf{84576}          & 84576.0         &  & \textbf{84576}   & 84576.0  \\
bmcp\_785\_800\_0.05\_2000    & 92431           & 92195.7  &  & 92608                  & 92482.7         &  & \textbf{92740}          & 92496.8         &  & \textbf{92740}   & 92624.4  \\
bmcp\_785\_800\_0.075\_1500   & 94245           & 94245.0  &  & \textbf{95221}         & 94835.2         &  & \textbf{95221}          & 94857.4         &  & \textbf{95221}   & 95221.0  \\
bmcp\_800\_785\_0.05\_2000    & 88562           & 88560.3  &  & \textbf{89138}         & 88984.7         &  & \textbf{89138}          & 89050.1         &  & \textbf{89138}   & 89094.7  \\
bmcp\_800\_785\_0.075\_1500   & 91021           & 90971.8  &  & \textbf{91856}         & 91404.0         &  & \textbf{91856}          & 91369.2         &  & \textbf{91856}   & 91722.0  \\
bmcp\_800\_800\_0.05\_2000    & 91748           & 90934.2  &  & \textbf{91795}         & 91601.2         &  & \textbf{91795}          & 91579.0         &  & \textbf{91795}   & 91679.1  \\
bmcp\_800\_800\_0.075\_1500   & 95533           & 95533.0  &  & \textbf{95995}         & 95307.8         &  & \textbf{95995}          & 95473.8         &  & \textbf{95995}   & 95653.8  \\
bmcp\_885\_900\_0.05\_2000    & 101293          & 101142.0 &  & \textbf{102277}        & 102020.1        &  & \textbf{102277}         & 102130.7        &  & \textbf{102277}  & 102140.6 \\
bmcp\_885\_900\_0.075\_1500   & 106364          & 105782.6 &  & \textbf{106940}        & 106463.7        &  & \textbf{106940}         & 106621.5        &  & \textbf{106940}  & 106477.2 \\
bmcp\_900\_885\_0.05\_2000    & 98840           & 98645.4  &  & \textbf{99590}         & 99288.2         &  & \textbf{99590}          & 99311.6         &  & \textbf{99590}   & 99397.4  \\
bmcp\_900\_885\_0.075\_1500   & \textbf{105141} & 103846.9 &  & \textbf{105141}        & 105041.4        &  & \textbf{105141}         & 104941.8        &  & \textbf{105141}  & 104991.6 \\
bmcp\_900\_900\_0.05\_2000    & 101265          & 101211.4 &  & \textbf{102055}        & 101673.8        &  & \textbf{102055}         & 101438.3        &  & \textbf{102055}  & 101464.8 \\
bmcp\_900\_900\_0.075\_1500   & 104521          & 104521.0 &  & 105041                 & 104781.0        &  & \textbf{105081}         & 104527.9        &  & \textbf{105081}  & 104966.0 \\
bmcp\_985\_1000\_0.05\_2000   & 109567          & 108938.0 &  & \textbf{110669}        & 109908.3        &  & \textbf{110669}         & 110571.0        &  & \textbf{110669}  & 109868.9 \\
bmcp\_985\_1000\_0.075\_1500  & 113541          & 113541.0 &  & \textbf{115505}        & 115004.2        &  & \textbf{115505}         & 114974.4        &  & \textbf{115505}  & 115080.3 \\
bmcp\_1000\_1000\_0.05\_2000  & 112640          & 111577.8 &  & \textbf{113331}        & 113047.4        &  & \textbf{113331}         & 113139.2        &  & \textbf{113331}  & 113131.8 \\
bmcp\_1000\_1000\_0.075\_1500 & 119453          & 118499.3 &  & \textbf{120246}        & 119923.4        &  & \textbf{120246}         & 120036.8        &  & \textbf{120246}  & 119954.1 \\
bmcp\_1000\_985\_0.05\_2000   & 111176          & 110712.6 &  & \textbf{112057}        & 111564.6        &  & 111859                  & 111590.0        &  & \textbf{112057}  & 111849.7 \\
bmcp\_1000\_985\_0.075\_1500  & 112250          & 112218.9 &  & \textbf{113615}        & 113287.4        &  & \textbf{113615}         & 112809.2        &  & \textbf{113615}  & 113104.5 \\ \hline
Average                       & 91733.9         & 91420.0  &  & 92284.8                & 91974.2         &  & 92272.9                 & 91988.4         &  & \textbf{92290.1} & 92039.3 \\ \bottomrule
\end{tabular}}
\end{table}

==> table_v5.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[b]
\centering
\caption{Comparison of the VDLS and its variant algorithms, VDLS$_{empty\_init}$ and VDLS$_{random\_init}$, as well as the PLTS algorithm, with 30 minutes of time limit in solving the 30 instances of the second set. Best results appear in bold.}
\label{table_v5}
\scalebox{0.6}{\begin{tabular}{lrrrrrrrrrrr} \toprule
\multirow{2}{*}{Instances}  & \multicolumn{2}{r}{PLTS}   &  & \multicolumn{2}{r}{VDLS$_{empty\_init}$} &  & \multicolumn{2}{r}{VDLS$_{random\_init}$} &  & \multicolumn{2}{r}{VDLS}     \\ \cline{2-3} \cline{5-6} \cline{8-9} \cline{11-12} 
                            & best            & average  &  & best                   & average         &  & best                    & average         &  & best              & average  \\ \hline
bmcp\_1100\_1000\_0.3\_3000 & 142835          & 142428.7 &  & \textbf{143475}        & 143206.0        &  & \textbf{143475}         & 143430.5        &  & 143402            & 143160.2 \\
bmcp\_1100\_1000\_0.5\_2000 & 125974          & 125790.0 &  & 127031                 & 126733.7        &  & \textbf{127157}         & 126749.6        &  & \textbf{127157}   & 126253.1 \\
bmcp\_1100\_1100\_0.3\_3000 & 154936          & 154661.7 &  & \textbf{157530}        & 156669.0        &  & 157264                  & 156466.4        &  & \textbf{157530}   & 156962.4 \\
bmcp\_1100\_1100\_0.5\_2000 & \textbf{139196} & 138169.0 &  & 139141                 & 138784.3        &  & \textbf{139196}         & 138798.4        &  & \textbf{139196}   & 138716.5 \\
bmcp\_1100\_1200\_0.3\_3000 & 169113          & 168763.6 &  & \textbf{172660}        & 171814.0        &  & \textbf{172660}         & 171902.5        &  & \textbf{172660}   & 172114.0 \\
bmcp\_1100\_1200\_0.5\_2000 & 150301          & 149366.4 &  & \textbf{150493}        & 150157.9        &  & \textbf{150493}         & 149934.0        &  & \textbf{150493}   & 150043.9 \\
bmcp\_1200\_1100\_0.3\_3000 & \textbf{161848} & 159620.3 &  & \textbf{161848}        & 161848.0        &  & \textbf{161848}         & 161848.0        &  & \textbf{161848}   & 161848.0 \\
bmcp\_1200\_1100\_0.5\_2000 & 135858          & 135509.2 &  & 137375                 & 136402.4        &  & 137365                  & 136545.0        &  & \textbf{137700}   & 136765.6 \\
bmcp\_1200\_1200\_0.3\_3000 & 169219          & 168821.7 &  & \textbf{172595}        & 171975.2        &  & \textbf{172595}         & 172233.5        &  & \textbf{172595}   & 172081.1 \\
bmcp\_1200\_1200\_0.5\_2000 & 149654          & 148679.1 &  & 150328                 & 149461.9        &  & \textbf{150850}         & 149311.2        &  & 149902            & 149334.4 \\
bmcp\_1200\_1300\_0.3\_3000 & 183004          & 182220.4 &  & \textbf{186083}        & 183817.7        &  & \textbf{186083}         & 184080.2        &  & 184431            & 183686.8 \\
bmcp\_1200\_1300\_0.5\_2000 & 160369          & 159735.4 &  & \textbf{162154}        & 161090.2        &  & 162029                  & 161047.0        &  & 161662            & 161074.5 \\
bmcp\_1300\_1200\_0.3\_3000 & 168586          & 168473.8 &  & 170372                 & 170049.4        &  & \textbf{170786}         & 169917.0        &  & 170283            & 169800.5 \\
bmcp\_1300\_1200\_0.5\_2000 & 151067          & 150034.7 &  & 151402                 & 150998.2        &  & 151402                  & 151024.4        &  & \textbf{151512}   & 151053.2 \\
bmcp\_1300\_1300\_0.3\_3000 & 180608          & 179978.4 &  & 184658                 & 183138.6        &  & 184366                  & 183187.5        &  & \textbf{184699}   & 183427.8 \\
bmcp\_1300\_1300\_0.5\_2000 & 160485          & 159511.3 &  & 162146                 & 161321.1        &  & \textbf{162189}         & 161175.1        &  & 162146            & 161523.8 \\
bmcp\_1300\_1400\_0.3\_3000 & 197709          & 195681.9 &  & \textbf{199134}        & 198784.3        &  & \textbf{199134}         & 198893.7        &  & \textbf{199134}   & 198913.4 \\
bmcp\_1300\_1400\_0.5\_2000 & 173349          & 171665.0 &  & 173666                 & 172733.4        &  & 173835                  & 173359.8        &  & \textbf{173954}   & 173773.5 \\
bmcp\_1400\_1300\_0.3\_3000 & 182881          & 180143.5 &  & 183914                 & 183682.4        &  & 183987                  & 183499.8        &  & \textbf{184148}   & 183536.2 \\
bmcp\_1400\_1300\_0.5\_2000 & 161995          & 160647.0 &  & 162378                 & 161537.8        &  & 162235                  & 161597.8        &  & \textbf{162544}   & 162324.7 \\
bmcp\_1400\_1400\_0.3\_3000 & 199879          & 197229.0 &  & 199883                 & 199582.9        &  & \textbf{200136}         & 199484.2        &  & \textbf{200136}   & 199714.5 \\
bmcp\_1400\_1400\_0.5\_2000 & 174683          & 173393.1 &  & 174265                 & 173609.7        &  & 174326                  & 173657.8        &  & \textbf{175583}   & 174370.2 \\
bmcp\_1400\_1500\_0.3\_3000 & 210077          & 208315.6 &  & 212327                 & 211205.6        &  & 211532                  & 211100.3        &  & \textbf{212492}   & 211356.6 \\
bmcp\_1400\_1500\_0.5\_2000 & 184259          & 183289.9 &  & 185902                 & 184583.7        &  & 186514                  & 184792.3        &  & \textbf{186818}   & 185991.7 \\
bmcp\_1500\_1400\_0.3\_3000 & 194156          & 193554.8 &  & \textbf{197899}        & 196925.1        &  & \textbf{197899}         & 196785.2        &  & \textbf{197899}   & 196753.8 \\
bmcp\_1500\_1400\_0.5\_2000 & 173475          & 171426.9 &  & 174284                 & 173741.9        &  & 174284                  & 173747.7        &  & \textbf{174522}   & 173745.1 \\
bmcp\_1500\_1500\_0.3\_3000 & 209929          & 207795.3 &  & \textbf{211108}        & 210405.7        &  & \textbf{211108}         & 210313.0        &  & \textbf{211108}   & 210451.1 \\
bmcp\_1500\_1500\_0.5\_2000 & 184082          & 182676.2 &  & \textbf{187052}        & 185367.7        &  & 185588                  & 184626.0        &  & \textbf{187052}   & 185464.7 \\
bmcp\_1500\_1600\_0.3\_3000 & \textbf{226408} & 221641.3 &  & \textbf{226408}        & 224383.9        &  & \textbf{226408}         & 224297.1        &  & \textbf{226408}   & 225031.9 \\
bmcp\_1500\_1600\_0.5\_2000 & 198214          & 196659.0 &  & 198686                 & 198049.4        &  & \textbf{198947}         & 198053.2        &  & 198579            & 198258.0 \\ \hline
Average                     & 172471.6        & 171196.1 &  & 173873.2               & 173068.7        &  & 173856.4                & 173061.9        &  & \textbf{173919.8} & 173251.0 \\ \bottomrule \vspace{-2em}
\end{tabular}}
\end{table}

==> table_v6.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[b]
\centering
\caption{Comparison of the VDLS and its variant algorithms, VDLS$_{empty\_init}$ and VDLS$_{random\_init}$, as well as the PLTS algorithm, with 30 minutes of time limit in solving the 30 instances of the third set. Best results appear in bold.}
\label{table_v6}
\scalebox{0.56}{\begin{tabular}{lrrrrrrrrrrr} \toprule
\multirow{2}{*}{Instances}   & \multicolumn{2}{r}{PLTS} &  & \multicolumn{2}{r}{VDLS$_{empty\_init}$} &  & \multicolumn{2}{r}{VDLS$_{random\_init}$} &  & \multicolumn{2}{r}{VDLS}       \\ \cline{2-3} \cline{5-6} \cline{8-9} \cline{11-12} 
                             & best        & average    &  & best                   & average         &  & best                    & average         &  & best               & average   \\ \hline
bmcp\_4200\_4000\_0.3\_10000 & 1778013     & 1747411.9  &  & 1831877                & 1803294.4       &  & 1831097                 & 1796122.4       &  & \textbf{1835947}   & 1828442.4 \\
bmcp\_4200\_4000\_0.5\_7000  & 1685141     & 1666673.3  &  & 1728603                & 1694691.7       &  & 1724315                 & 1699145.8       &  & \textbf{1733033}   & 1724198.8 \\
bmcp\_4200\_4200\_0.3\_10000 & 1874190     & 1839780.1  &  & 1914893                & 1891892.3       &  & 1916604                 & 1885356.8       &  & \textbf{1922985}   & 1915332.4 \\
bmcp\_4200\_4200\_0.5\_7000  & 1764277     & 1742121.7  &  & 1789094                & 1764485.7       &  & 1800408                 & 1770795.1       &  & \textbf{1802880}   & 1798430.9 \\
bmcp\_4200\_4400\_0.3\_10000 & 1954069     & 1932251.0  &  & 2015247                & 1974028.3       &  & \textbf{2022834}        & 1975630.2       &  & \textbf{2022834}   & 2016260.1 \\
bmcp\_4200\_4400\_0.5\_7000  & 1853677     & 1820444.4  &  & 1884460                & 1851526.5       &  & \textbf{1897148}        & 1853408.6       &  & 1894307            & 1883721.0 \\
bmcp\_4400\_4200\_0.3\_10000 & 1833465     & 1816879.1  &  & 1883442                & 1869600.9       &  & 1878799                 & 1868611.8       &  & \textbf{1911617}   & 1905971.7 \\
bmcp\_4400\_4200\_0.5\_7000  & 1746064     & 1730783.9  &  & 1792406                & 1768577.0       &  & 1767535                 & 1760287.7       &  & \textbf{1807860}   & 1799645.5 \\
bmcp\_4400\_4400\_0.3\_10000 & 1945218     & 1922134.2  &  & 2020371                & 1983709.5       &  & 2014130                 & 1983868.2       &  & \textbf{2023432}   & 2019636.3 \\
bmcp\_4400\_4400\_0.5\_7000  & 1844031     & 1821467.8  &  & 1892872                & 1855345.7       &  & \textbf{1903551}        & 1857785.4       &  & 1888693            & 1882463.1 \\
bmcp\_4400\_4600\_0.3\_10000 & 2003959     & 1993946.2  &  & 2050043                & 2044121.7       &  & 2089880                 & 2050780.2       &  & \textbf{2097123}   & 2088349.1 \\
bmcp\_4400\_4600\_0.5\_7000  & 1937066     & 1906956.1  &  & 1975949                & 1944492.3       &  & 1973323                 & 1949916.7       &  & \textbf{1981337}   & 1973941.3 \\
bmcp\_4600\_4400\_0.3\_10000 & 1930498     & 1913501.0  &  & 1961826                & 1955179.3       &  & 1964666                 & 1958934.3       &  & \textbf{2011730}   & 1998707.0 \\
bmcp\_4600\_4400\_0.5\_7000  & 1845046     & 1817697.2  &  & 1876239                & 1853602.3       &  & 1892043                 & 1855062.5       &  & \textbf{1897119}   & 1889599.7 \\
bmcp\_4600\_4600\_0.3\_10000 & 2027132     & 2005096.7  &  & \textbf{2104132}       & 2056387.5       &  & 2061350                 & 2049326.1       &  & 2103476            & 2093832.3 \\
bmcp\_4600\_4600\_0.5\_7000  & 1921261     & 1900376.3  &  & 1962586                & 1937715.7       &  & 1961824                 & 1938126.8       &  & \textbf{1976832}   & 1970554.1 \\
bmcp\_4600\_4800\_0.3\_10000 & 2120120     & 2091722.5  &  & 2191184                & 2157173.4       &  & 2194985                 & 2168282.3       &  & \textbf{2200580}   & 2193619.0 \\
bmcp\_4600\_4800\_0.5\_7000  & 1989454     & 1967943.3  &  & 2054827                & 2033259.2       &  & 2057415                 & 2021947.2       &  & \textbf{2064098}   & 2053550.3 \\
bmcp\_4800\_4600\_0.3\_10000 & 2019033     & 1991673.5  &  & 2087870                & 2052936.6       &  & \textbf{2095843}        & 2045652.0       &  & 2093497            & 2081197.6 \\
bmcp\_4800\_4600\_0.5\_7000  & 1922466     & 1901157.6  &  & 1954551                & 1931919.1       &  & 1970388                 & 1945618.6       &  & \textbf{1977557}   & 1969484.1 \\
bmcp\_4800\_4800\_0.3\_10000 & 2100773     & 2058921.6  &  & 2178066                & 2124181.1       &  & 2163574                 & 2129659.4       &  & \textbf{2180165}   & 2171120.6 \\
bmcp\_4800\_4800\_0.5\_7000  & 2009129     & 1973993.6  &  & 2052047                & 2025585.3       &  & \textbf{2061157}        & 2022687.2       &  & 2058797            & 2053170.9 \\
bmcp\_4800\_5000\_0.3\_10000 & 2184445     & 2157793.0  &  & 2267237                & 2230084.3       &  & 2271401                 & 2221344.3       &  & \textbf{2275455}   & 2270224.7 \\
bmcp\_4800\_5000\_0.5\_7000  & 2087596     & 2050741.0  &  & \textbf{2136422}       & 2094032.4       &  & 2129092                 & 2092725.4       &  & 2133843            & 2129594.0 \\
bmcp\_5000\_4800\_0.3\_10000 & 2069979     & 2051607.2  &  & 2179786                & 2125879.6       &  & 2179343                 & 2123597.7       &  & \textbf{2181584}   & 2167254.8 \\
bmcp\_5000\_4800\_0.5\_7000  & 2013921     & 1977310.7  &  & 2057167                & 2033632.2       &  & 2023965                 & 2008655.9       &  & \textbf{2061909}   & 2053025.7 \\
bmcp\_5000\_5000\_0.3\_10000 & 2144223     & 2126462.9  &  & 2245140                & 2199261.0       &  & 2201533                 & 2191866.8       &  & \textbf{2254007}   & 2247746.1 \\
bmcp\_5000\_5000\_0.5\_7000  & 2067188     & 2046886.5  &  & 2138756                & 2097677.8       &  & 2131933                 & 2093120.8       &  & \textbf{2145927}   & 2135823.3 \\
bmcp\_5000\_5200\_0.3\_10000 & 2231359     & 2220887.2  &  & 2290213                & 2279731.0       &  & 2346931                 & 2298733.8       &  & \textbf{2352676}   & 2340288.0 \\
bmcp\_5000\_5200\_0.5\_7000  & 2129556     & 2115338.3  &  & 2205192                & 2170351.3       &  & 2203467                 & 2175096.1       &  & \textbf{2224001}   & 2207572.4 \\ \hline
Average                      & 1967745.0   & 1943665.3  &  & 2024083.3              & 1993478.5       &  & 2024351.1               & 1993071.5       &  & \textbf{2037176.7} & 2028758.6 \\ \bottomrule \vspace{-2em}
\end{tabular}}
\end{table}

==> tables/table1-10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[b]
\centering
\caption{Comparison of the PLTS and VDLS with both 10 minutes of time limit, and the CPLEX solver with 2 hours and 5 hours of time limit in solving the 30 instances of the first set. Best results appear in bold.}
\label{table1-10}
\scalebox{0.56}{\begin{tabular}{lrrrrrrrrrrr} \toprule
\multirow{2}{*}{Instances}    & \multicolumn{2}{r}{CPLEX(2 hours)} & \multicolumn{1}{l}{} & \multicolumn{2}{r}{CPLEX(5 hours)} & \multicolumn{1}{l}{} & \multicolumn{2}{r}{PLTS}  &  & \multicolumn{2}{r}{VDLS}    \\ \cline{2-3} \cline{5-6} \cline{8-9} \cline{11-12} 
                              & LB              & UB               & \multicolumn{1}{l}{} & LB              & UB               & \multicolumn{1}{l}{} & best           & average  &  & best             & average  \\ \hline
bmcp\_585\_600\_0.05\_2000    & 67910           & 73495.9          &                      & 70742           & 74224.9          &                      & 70997          & 70892.6  &  & \textbf{71102}   & 71034.4  \\
bmcp\_585\_600\_0.075\_1500   & 68418           & 77549.4          &                      & 69172           & 76716.9          &                      & 70677          & 70535.9  &  & \textbf{71025}   & 70492.5  \\
bmcp\_600\_585\_0.05\_2000    & 66184           & 71739.7          &                      & 66452           & 71094.3          &                      & 67187          & 66807.1  &  & \textbf{67636}   & 67621.6  \\
bmcp\_600\_585\_0.075\_1500   & 68145           & 77321.5          &                      & 70113           & 76332.9          &                      & 70318          & 70318.0  &  & \textbf{70588}   & 70277.0  \\
bmcp\_600\_600\_0.05\_2000    & 67917           & 73495.1          &                      & 68477           & 72880.9          &                      & 68453          & 68346.6  &  & \textbf{68738}   & 68580.7  \\
bmcp\_600\_600\_0.075\_1500   & 70947           & 77380.0          &                      & 71018           & 76337.7          &                      & 71746          & 71746.0  &  & \textbf{71904}   & 71780.7  \\
bmcp\_685\_700\_0.05\_2000    & 79997           & 88954.3          &                      & 80783           & 88447.7          &                      & 80111          & 79979.9  &  & \textbf{81227}   & 80482.5  \\
bmcp\_685\_700\_0.075\_1500   & 80443           & 92328.3          &                      & 81639           & 91379.0          &                      & 82955          & 82933.4  &  & \textbf{83286}   & 82886.6  \\
bmcp\_700\_685\_0.05\_2000    & 76139           & 83561.9          &                      & 77176           & 82815.1          &                      & \textbf{78054} & 77460.8  &  & \textbf{78054}   & 77742.9  \\
bmcp\_700\_685\_0.075\_1500   & 75841           & 86956.9          &                      & 76033           & 86566.8          &                      & \textbf{78869} & 78580.1  &  & \textbf{78869}   & 78642.9  \\
bmcp\_700\_700\_0.05\_2000    & 76367           & 85587.3          &                      & 77056           & 84855.4          &                      & 77424          & 77225.8  &  & \textbf{78458}   & 78180.4  \\
bmcp\_700\_700\_0.075\_1500   & 81645           & 93026.7          &                      & 81645           & 92152.0          &                      & 84570          & 83406.5  &  & \textbf{84576}   & 84576.0  \\
bmcp\_785\_800\_0.05\_2000    & 90705           & 102198.7         &                      & 91319           & 101585.7         &                      & 92505          & 92080.7  &  & \textbf{92740}   & 92414.2  \\
bmcp\_785\_800\_0.075\_1500   & 92358           & 107354.5         &                      & 92358           & 106842.7         &                      & 94245          & 94243.8  &  & \textbf{95221}   & 95221.0  \\
bmcp\_800\_785\_0.05\_2000    & 86139           & 97891.1          &                      & 86813           & 97477.3          &                      & 88562          & 88424.3  &  & \textbf{89138}   & 89054.7  \\
bmcp\_800\_785\_0.075\_1500   & 89018           & 103644.1         &                      & 89229           & 102868.0         &                      & 91021          & 90888.9  &  & \textbf{91856}   & 91722.9  \\
bmcp\_800\_800\_0.05\_2000    & 90344           & 101141.0         &                      & 89872           & 100373.8         &                      & 90951          & 90697.4  &  & \textbf{91795}   & 91572.8  \\
bmcp\_800\_800\_0.075\_1500   & 94049           & 108713.0         &                      & 94049           & 108005.6         &                      & 95533          & 95508.8  &  & \textbf{95995}   & 95568.5  \\
bmcp\_885\_900\_0.05\_2000    & 100085          & 114313.8         &                      & 99845           & 113747.0         &                      & 101293         & 100857.0 &  & \textbf{102277}  & 102059.2 \\
bmcp\_885\_900\_0.075\_1500   & 102423          & 122684.4         &                      & 102933          & 122093.5         &                      & 105718         & 105707.7 &  & \textbf{106940}  & 106446.9 \\
bmcp\_900\_885\_0.05\_2000    & 97088           & 110828.8         &                      & 96945           & 109948.5         &                      & 98840          & 98485.5  &  & \textbf{99590}   & 99365.1  \\
bmcp\_900\_885\_0.075\_1500   & 99881           & 119045.5         &                      & 99888           & 118554.8         &                      & 103596         & 103223.1 &  & \textbf{105141}  & 105024.8 \\
bmcp\_900\_900\_0.05\_2000    & 100108          & 115682.6         &                      & 100412          & 114551.1         &                      & 101265         & 101210.7 &  & \textbf{102055}  & 101402.6 \\
bmcp\_900\_900\_0.075\_1500   & 101035          & 120452.8         &                      & 99888           & 118554.8         &                      & 104521         & 104521.0 &  & \textbf{105081}  & 104919.1 \\
bmcp\_985\_1000\_0.05\_2000   & 107820          & 125903.7         &                      & 107488          & 124487.4         &                      & 109523         & 108681.8 &  & \textbf{110669}  & 109792.6 \\
bmcp\_985\_1000\_0.075\_1500  & 110769          & 134440.4         &                      & 111177          & 133789.8         &                      & 113541         & 113439.4 &  & \textbf{115505}  & 114765.3 \\
bmcp\_1000\_985\_0.05\_2000   & 108714          & 126779.1         &                      & 110134          & 125574.8         &                      & 111212         & 110379.1 &  & \textbf{112057}  & 111583.1 \\
bmcp\_1000\_985\_0.075\_1500  & 108801          & 131873.0         &                      & 108801          & 130981.4         &                      & 112250         & 112160.2 &  & \textbf{113615}  & 113096.1 \\
bmcp\_1000\_1000\_0.05\_2000  & 109928          & 131194.2         &                      & 111155          & 128583.6         &                      & 111829         & 111318.6 &  & \textbf{113331}  & 113124.8 \\
bmcp\_1000\_1000\_0.075\_1500 & 115313          & 139152.9         &                      & 115824          & 137900.4         &                      & 118244         & 118243.1 &  & \textbf{120246}  & 119994.5 \\ \hline
Average                       & 89484.4         & 103156.3         &                      & 89947.9         & 102324.1         &                      & 91533.7        & 91276.8  &  & \textbf{92290.5} & 91980.9 
      \\ \bottomrule              
\end{tabular}}
\end{table}

==> tables/table1-30.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\caption{Comparison of the PLTS and VDLS with both 30 minutes of time limit, and the CPLEX solver with 2 hours and 5 hours of time limit in solving the 30 instances of the first set. Best results appear in bold.}
\label{table1-30}
\scalebox{0.56}{\begin{tabular}{lrrrrrrrrrrr} \toprule
\multirow{2}{*}{Instances}    & \multicolumn{2}{r}{CPLEX(2 hours)} & \multicolumn{1}{l}{} & \multicolumn{2}{r}{CPLEX(5 hours)} & \multicolumn{1}{l}{} & \multicolumn{2}{r}{PLTS}   &  & \multicolumn{2}{r}{VDLS}                       \\ \cline{2-3} \cline{5-6} \cline{8-9} \cline{11-12} 
                              & LB              & UB               & \multicolumn{1}{l}{} & LB              & UB               & \multicolumn{1}{l}{} & best            & average  &  & best             & \multicolumn{1}{r}{average} \\ \hline
bmcp\_585\_600\_0.05\_2000    & 67910           & 73495.9          &                      & 70742           & 74224.9          &                      & \textbf{71102}  & 70915.0  &  & \textbf{71102}   & 71034.4                     \\
bmcp\_585\_600\_0.075\_1500   & 68418           & 77549.4          &                      & 69172           & 76716.9          &                      & 70677           & 70670.2  &  & \textbf{71025}   & 70492.5                     \\
bmcp\_600\_585\_0.05\_2000    & 66184           & 71739.7          &                      & 66452           & 71094.3          &                      & \textbf{67636}  & 67041.5  &  & \textbf{67636}   & 67621.6                     \\
bmcp\_600\_585\_0.075\_1500   & 68145           & 77321.5          &                      & 70113           & 76332.9          &                      & 70318           & 70318.0  &  & \textbf{70588}   & 70277.0                     \\
bmcp\_600\_600\_0.05\_2000    & 67917           & 73495.1          &                      & 68477           & 72880.9          &                      & 68453           & 68386.8  &  & \textbf{68738}   & 68580.7                     \\
bmcp\_600\_600\_0.075\_1500   & 70947           & 77380.0          &                      & 71018           & 76337.7          &                      & 71746           & 71746.0  &  & \textbf{71904}   & 71780.7                     \\
bmcp\_685\_700\_0.05\_2000    & 79997           & 88954.3          &                      & 80783           & 88447.7          &                      & 80197           & 80096.6  &  & \textbf{81227}   & 80482.5                     \\
bmcp\_685\_700\_0.075\_1500   & 80443           & 92328.3          &                      & 81639           & 91379.0          &                      & 82955           & 82944.2  &  & \textbf{83286}   & 82886.6                     \\
bmcp\_700\_685\_0.05\_2000    & 76139           & 83561.9          &                      & 77176           & 82815.1          &                      & 77876           & 77372.7  &  & \textbf{78054}   & 77742.9                     \\
bmcp\_700\_685\_0.075\_1500   & 75841           & 86956.9          &                      & 76033           & 86566.8          &                      & \textbf{78869}  & 78810.4  &  & \textbf{78869}   & 78642.9                     \\
bmcp\_700\_700\_0.05\_2000    & 76367           & 85587.3          &                      & 77056           & 84855.4          &                      & 78028           & 77501.5  &  & \textbf{78458}   & 78200.7                     \\
bmcp\_700\_700\_0.075\_1500   & 81645           & 93026.7          &                      & 81645           & 92152.0          &                      & 84570           & 83720.7  &  & \textbf{84576}   & 84576.0                     \\
bmcp\_785\_800\_0.05\_2000    & 90705           & 102198.7         &                      & 91319           & 101585.7         &                      & 92431           & 92195.7  &  & \textbf{92740}   & 92419.7                     \\
bmcp\_785\_800\_0.075\_1500   & 92358           & 107354.5         &                      & 92358           & 106842.7         &                      & 94245           & 94245.0  &  & \textbf{95221}   & 95221.0                     \\
bmcp\_800\_785\_0.05\_2000    & 86139           & 97891.1          &                      & 86813           & 97477.3          &                      & 88562           & 88560.3  &  & \textbf{89138}   & 89054.7                     \\
bmcp\_800\_785\_0.075\_1500   & 89018           & 103644.1         &                      & 89229           & 102868.0         &                      & 91021           & 90971.8  &  & \textbf{91856}   & 91722.9                     \\
bmcp\_800\_800\_0.05\_2000    & 90344           & 101141.0         &                      & 89872           & 100373.8         &                      & 91748           & 90934.2  &  & \textbf{91795}   & 91604.5                     \\
bmcp\_800\_800\_0.075\_1500   & 94049           & 108713.0         &                      & 94049           & 108005.6         &                      & 95533           & 95533.0  &  & \textbf{95995}   & 95568.5                     \\
bmcp\_885\_900\_0.05\_2000    & 100085          & 114313.8         &                      & 99845           & 113747.0         &                      & 101293          & 101142.0 &  & \textbf{102277}  & 102059.2                    \\
bmcp\_885\_900\_0.075\_1500   & 102423          & 122684.4         &                      & 102933          & 122093.5         &                      & 106364          & 105782.6 &  & \textbf{106940}  & 106446.9                    \\
bmcp\_900\_885\_0.05\_2000    & 97088           & 110828.8         &                      & 96945           & 109948.5         &                      & 98840           & 98645.4  &  & \textbf{99590}   & 99368.7                     \\
bmcp\_900\_885\_0.075\_1500   & 99881           & 119045.5         &                      & 99888           & 118554.8         &                      & \textbf{105141} & 103846.9 &  & \textbf{105141}  & 105024.8                    \\
bmcp\_900\_900\_0.05\_2000    & 100108          & 115682.6         &                      & 100412          & 114551.1         &                      & 101265          & 101211.4 &  & \textbf{102055}  & 101481.4                    \\
bmcp\_900\_900\_0.075\_1500   & 101035          & 120452.8         &                      & 99888           & 118554.8         &                      & 104521          & 104521.0 &  & \textbf{105081}  & 104919.1                    \\
bmcp\_985\_1000\_0.05\_2000   & 107820          & 125903.7         &                      & 107488          & 124487.4         &                      & 109567          & 108938.0 &  & \textbf{110669}  & 109792.6                    \\
bmcp\_985\_1000\_0.075\_1500  & 110769          & 134440.4         &                      & 111177          & 133789.8         &                      & 113541          & 113541.0 &  & \textbf{115505}  & 114765.3                    \\
bmcp\_1000\_985\_0.05\_2000   & 109928          & 131194.2         &                      & 111155          & 128583.6         &                      & 111176          & 110712.6 &  & \textbf{112057}  & 111624.7                    \\
bmcp\_1000\_985\_0.075\_1500  & 115313          & 139152.9         &                      & 115824          & 137900.4         &                      & 112250          & 112218.9 &  & \textbf{113615}  & 113096.1                    \\
bmcp\_1000\_1000\_0.05\_2000  & 108714          & 126779.1         &                      & 110134          & 125574.8         &                      & 112640          & 111577.8 &  & \textbf{113331}  & 113129.6                    \\
bmcp\_1000\_1000\_0.075\_1500 & 108801          & 131873.0         &                      & 108801          & 130981.4         &                      & 119453          & 118499.3 &  & \textbf{120246}  & 119994.5                    \\ \hline
Average                       & 89484.4         & 103156.3         &                      & 89947.9         & 102324.1         &                      & 91733.9         & 91420.0  &  & \textbf{92290.5} & 91987.1                    \\ \bottomrule
\end{tabular}}
\end{table}

==> tables/table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\caption{Comparison results of VDLS and PLTS, with 10 or 30 minutes of time limit, on the 30 instances of the second set. Best results appear in bold.}
\label{table2}
\scalebox{0.65}{\begin{tabular}{lrrrrr} \toprule
\multirow{2}{*}{Instances}  & \multicolumn{2}{r}{PLTS}   &  & \multicolumn{2}{r}{VDLS}     \\ \cline{2-3} \cline{5-6} 
                            & best            & average  &  & best              & average  \\ \hline
\multicolumn{6}{l}{10 minutes of time limit}                                               \\ \hline
bmcp\_1100\_1000\_0.3\_3000 & 142574          & 141985.1 &  & \textbf{143475}   & 143222.1 \\
bmcp\_1100\_1000\_0.5\_2000 & 125790          & 125479.5 &  & \textbf{126582}   & 125970.4 \\
bmcp\_1100\_1100\_0.3\_3000 & 154726          & 153867.0 &  & \textbf{157530}   & 156462.5 \\
bmcp\_1100\_1100\_0.5\_2000 & 138160          & 137490.0 &  & \textbf{139141}   & 138694.5 \\
bmcp\_1100\_1200\_0.3\_3000 & 169980          & 168661.8 &  & \textbf{172660}   & 172075.3 \\
bmcp\_1100\_1200\_0.5\_2000 & 149402          & 148618.4 &  & \textbf{150493}   & 149860.2 \\
bmcp\_1200\_1100\_0.3\_3000 & \textbf{161848} & 159267.2 &  & \textbf{161848}   & 161817.3 \\
bmcp\_1200\_1100\_0.5\_2000 & 136073          & 135347.1 &  & \textbf{137700}   & 136564.8 \\
bmcp\_1200\_1200\_0.3\_3000 & 169219          & 168710.1 &  & \textbf{172595}   & 172095.7 \\
bmcp\_1200\_1200\_0.5\_2000 & 148706          & 147717.1 &  & \textbf{151440}   & 149480.5 \\
bmcp\_1200\_1300\_0.3\_3000 & 184156          & 181891.2 &  & \textbf{184384}   & 183583.0 \\
bmcp\_1200\_1300\_0.5\_2000 & 160487          & 159181.1 &  & \textbf{162154}   & 160955.4 \\
bmcp\_1300\_1200\_0.3\_3000 & 168304          & 167883.9 &  & \textbf{170786}   & 169724.7 \\
bmcp\_1300\_1200\_0.5\_2000 & 150249          & 148937.0 &  & \textbf{151402}   & 150995.1 \\
bmcp\_1300\_1300\_0.3\_3000 & 180593          & 179909.5 &  & \textbf{184699}   & 183180.9 \\
bmcp\_1300\_1300\_0.5\_2000 & 160677          & 159351.7 &  & \textbf{162146}   & 161493.6 \\
bmcp\_1300\_1400\_0.3\_3000 & 195341          & 195308.4 &  & \textbf{199134}   & 198818.9 \\
bmcp\_1300\_1400\_0.5\_2000 & 172244          & 171175.5 &  & \textbf{173954}   & 173718.2 \\
bmcp\_1400\_1300\_0.3\_3000 & 181154          & 179794.4 &  & \textbf{183987}   & 183792.4 \\
bmcp\_1400\_1300\_0.5\_2000 & 161658          & 159182.6 &  & \textbf{162544}   & 162190.5 \\
bmcp\_1400\_1400\_0.3\_3000 & 199067          & 197227.7 &  & \textbf{200136}   & 199593.2 \\
bmcp\_1400\_1400\_0.5\_2000 & 173693          & 172899.6 &  & \textbf{175324}   & 173898.9 \\
bmcp\_1400\_1500\_0.3\_3000 & 210450          & 208051.0 &  & \textbf{212492}   & 211196.8 \\
bmcp\_1400\_1500\_0.5\_2000 & 183146          & 182427.8 &  & \textbf{186818}   & 186118.5 \\
bmcp\_1500\_1400\_0.3\_3000 & 193676          & 192820.3 &  & \textbf{197219}   & 196642.5 \\
bmcp\_1500\_1400\_0.5\_2000 & 171949          & 170581.2 &  & \textbf{174284}   & 173461.7 \\
bmcp\_1500\_1500\_0.3\_3000 & 208630          & 206404.9 &  & \textbf{211108}   & 210222.4 \\
bmcp\_1500\_1500\_0.5\_2000 & 183599          & 181456.4 &  & \textbf{187052}   & 184938.1 \\
bmcp\_1500\_1600\_0.3\_3000 & \textbf{226408} & 221501.2 &  & \textbf{226408}   & 224514.1 \\
bmcp\_1500\_1600\_0.5\_2000 & 197566          & 195828.2 &  & \textbf{198663}   & 198137.0 \\ \hline
Average                     & 171984.2        & 170631.9 &  & \textbf{173938.6} & 173114.0 \\ \hline
\multicolumn{6}{l}{30 minutes of time limit}                                               \\ \hline
bmcp\_1100\_1000\_0.3\_3000 & 142835          & 142428.7 &  & \textbf{143475}   & 143224.6 \\
bmcp\_1100\_1000\_0.5\_2000 & 125974          & 125790.0 &  & \textbf{126917}   & 126021.6 \\
bmcp\_1100\_1100\_0.3\_3000 & 154936          & 154661.7 &  & \textbf{157530}   & 156462.5 \\
bmcp\_1100\_1100\_0.5\_2000 & \textbf{139196} & 138169.0 &  & 139141            & 138719.4 \\
bmcp\_1100\_1200\_0.3\_3000 & 169113          & 168763.6 &  & \textbf{172660}   & 172075.3 \\
bmcp\_1100\_1200\_0.5\_2000 & 150301          & 149366.4 &  & \textbf{150493}   & 149944.0 \\
bmcp\_1200\_1100\_0.3\_3000 & \textbf{161848} & 159620.3 &  & \textbf{161848}   & 161848.0 \\
bmcp\_1200\_1100\_0.5\_2000 & 135858          & 135509.2 &  & \textbf{137700}   & 136831.2 \\
bmcp\_1200\_1200\_0.3\_3000 & 169219          & 168821.7 &  & \textbf{172595}   & 172151.8 \\
bmcp\_1200\_1200\_0.5\_2000 & 149654          & 148679.1 &  & \textbf{151440}   & 149610.0 \\
bmcp\_1200\_1300\_0.3\_3000 & 183004          & 182220.4 &  & \textbf{186083}   & 183599.0 \\
bmcp\_1200\_1300\_0.5\_2000 & 160369          & 159735.4 &  & \textbf{162154}   & 161146.9 \\
bmcp\_1300\_1200\_0.3\_3000 & 168586          & 168473.8 &  & \textbf{170786}   & 169724.7 \\
bmcp\_1300\_1200\_0.5\_2000 & 151067          & 150034.7 &  & \textbf{151402}   & 151049.4 \\
bmcp\_1300\_1300\_0.3\_3000 & 180608          & 179978.4 &  & \textbf{184699}   & 183239.0 \\
bmcp\_1300\_1300\_0.5\_2000 & 160485          & 159511.3 &  & \textbf{162146}   & 161536.7 \\
bmcp\_1300\_1400\_0.3\_3000 & 197709          & 195681.9 &  & \textbf{199134}   & 198889.4 \\
bmcp\_1300\_1400\_0.5\_2000 & 173349          & 171665.0 &  & \textbf{173954}   & 173799.2 \\
bmcp\_1400\_1300\_0.3\_3000 & 182881          & 180143.5 &  & \textbf{183987}   & 183796.3 \\
bmcp\_1400\_1300\_0.5\_2000 & 161995          & 160647.0 &  & \textbf{162544}   & 162312.9 \\
bmcp\_1400\_1400\_0.3\_3000 & 199879          & 197229.0 &  & \textbf{200136}   & 199616.7 \\
bmcp\_1400\_1400\_0.5\_2000 & 174683          & 173393.1 &  & \textbf{175583}   & 173984.9 \\
bmcp\_1400\_1500\_0.3\_3000 & 210077          & 208315.6 &  & \textbf{212492}   & 211264.4 \\
bmcp\_1400\_1500\_0.5\_2000 & 184259          & 183289.9 &  & \textbf{186818}   & 186250.3 \\
bmcp\_1500\_1400\_0.3\_3000 & 194156          & 193554.8 &  & \textbf{197219}   & 196703.4 \\
bmcp\_1500\_1400\_0.5\_2000 & 173475          & 171426.9 &  & \textbf{174284}   & 173576.4 \\
bmcp\_1500\_1500\_0.3\_3000 & 209929          & 207795.3 &  & \textbf{211108}   & 210393.7 \\
bmcp\_1500\_1500\_0.5\_2000 & 184082          & 182676.2 &  & \textbf{187052}   & 185221.6 \\
bmcp\_1500\_1600\_0.3\_3000 & \textbf{226408} & 221641.3 &  & \textbf{226408}   & 224926.6 \\
bmcp\_1500\_1600\_0.5\_2000 & 198214          & 196659.0 &  & \textbf{199678}   & 198462.6 \\ \hline
Average                     & 172471.6        & 171196.1 &  & \textbf{174048.9} & 173212.8 \\ \bottomrule
\end{tabular}}
\end{table}

==> tables/table3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\caption{Comparison results of VDLS and PLTS, with 10 or 30 minutes of time limit, on the 30 instances of the third set. Best results appear in bold.}
\label{table3}
\scalebox{0.65}{\begin{tabular}{lrrrrr} \toprule
\multirow{2}{*}{Instances}   & \multicolumn{2}{r}{PLTS} &  & \multicolumn{2}{r}{VDLS}       \\ \cline{2-3} \cline{5-6} 
                             & best        & average    &  & best               & average   \\ \hline
\multicolumn{6}{l}{10 minutes of time limit}                                                \\ \hline
bmcp\_4200\_4000\_0.3\_10000 & 1775432     & 1736438.9  &  & \textbf{1835947}   & 1827846.2 \\
bmcp\_4200\_4000\_0.5\_7000  & 1692056     & 1662063.5  &  & \textbf{1735128}   & 1720514.4 \\
bmcp\_4200\_4200\_0.3\_10000 & 1856948     & 1824810.6  &  & \textbf{1924499}   & 1912643.9 \\
bmcp\_4200\_4200\_0.5\_7000  & 1759417     & 1735178.9  &  & \textbf{1801634}   & 1796598.8 \\
bmcp\_4200\_4400\_0.3\_10000 & 1964294     & 1928237.3  &  & \textbf{2021037}   & 2015973.6 \\
bmcp\_4200\_4400\_0.5\_7000  & 1846157     & 1815658.3  &  & \textbf{1893350}   & 1883659.3 \\
bmcp\_4400\_4200\_0.3\_10000 & 1817604     & 1797114.8  &  & \textbf{1914670}   & 1905583.0 \\
bmcp\_4400\_4200\_0.5\_7000  & 1762870     & 1724377.3  &  & \textbf{1807499}   & 1800460.9 \\
bmcp\_4400\_4400\_0.3\_10000 & 1948267     & 1918148.4  &  & \textbf{2026134}   & 2017604.4 \\
bmcp\_4400\_4400\_0.5\_7000  & 1817416     & 1806039.0  &  & \textbf{1893155}   & 1880770.0 \\
bmcp\_4400\_4600\_0.3\_10000 & 2016242     & 1989001.0  &  & \textbf{2096767}   & 2086931.0 \\
bmcp\_4400\_4600\_0.5\_7000  & 1913938     & 1895993.0  &  & \textbf{1985446}   & 1973491.3 \\
bmcp\_4600\_4400\_0.3\_10000 & 1939966     & 1894543.2  &  & \textbf{2005469}   & 1995349.8 \\
bmcp\_4600\_4400\_0.5\_7000  & 1822083     & 1803727.3  &  & \textbf{1891961}   & 1886326.4 \\
bmcp\_4600\_4600\_0.3\_10000 & 2027745     & 1996365.4  &  & \textbf{2103062}   & 2093885.6 \\
bmcp\_4600\_4600\_0.5\_7000  & 1932145     & 1886756.8  &  & \textbf{1977544}   & 1967468.6 \\
bmcp\_4600\_4800\_0.3\_10000 & 2090814     & 2062236.5  &  & \textbf{2199773}   & 2188595.1 \\
bmcp\_4600\_4800\_0.5\_7000  & 2006997     & 1964777.6  &  & \textbf{2059987}   & 2051531.7 \\
bmcp\_4800\_4600\_0.3\_10000 & 2008566     & 1974395.8  &  & \textbf{2088967}   & 2080467.4 \\
bmcp\_4800\_4600\_0.5\_7000  & 1902428     & 1879771.0  &  & \textbf{1975756}   & 1966373.7 \\
bmcp\_4800\_4800\_0.3\_10000 & 2071733     & 2034925.5  &  & \textbf{2180765}   & 2168243.6 \\
bmcp\_4800\_4800\_0.5\_7000  & 1981902     & 1955184.4  &  & \textbf{2063921}   & 2053363.9 \\
bmcp\_4800\_5000\_0.3\_10000 & 2221536     & 2157486.8  &  & \textbf{2274851}   & 2269242.4 \\
bmcp\_4800\_5000\_0.5\_7000  & 2055213     & 2032723.9  &  & \textbf{2139652}   & 2128574.9 \\
bmcp\_5000\_4800\_0.3\_10000 & 2076374     & 2039438.7  &  & \textbf{2179552}   & 2166424.9 \\
bmcp\_5000\_4800\_0.5\_7000  & 1987069     & 1962373.3  &  & \textbf{2057220}   & 2049177.5 \\
bmcp\_5000\_5000\_0.3\_10000 & 2154362     & 2103199.9  &  & \textbf{2255867}   & 2245749.3 \\
bmcp\_5000\_5000\_0.5\_7000  & 2077170     & 2041834.9  &  & \textbf{2146446}   & 2134731.1 \\
bmcp\_5000\_5200\_0.3\_10000 & 2235890     & 2211542.6  &  & \textbf{2347464}   & 2337836.8 \\
bmcp\_5000\_5200\_0.5\_7000  & 2119204     & 2099244.2  &  & \textbf{2218955}   & 2205056.8 \\ \hline
Average                      & 1962727.9   & 1931119.6  &  & \textbf{2036749.3} & 2027015.9 \\ \hline
\multicolumn{6}{l}{30 minutes of time limit}                                                \\ \hline
bmcp\_4200\_4000\_0.3\_10000 & 1778013     & 1747411.9  &  & \textbf{1835947}   & 1833108.2 \\
bmcp\_4200\_4000\_0.5\_7000  & 1685141     & 1666673.3  &  & \textbf{1738553}   & 1729188.0 \\
bmcp\_4200\_4200\_0.3\_10000 & 1874190     & 1839780.1  &  & \textbf{1925706}   & 1918624.2 \\
bmcp\_4200\_4200\_0.5\_7000  & 1764277     & 1742121.7  &  & \textbf{1811649}   & 1801880.2 \\
bmcp\_4200\_4400\_0.3\_10000 & 1954069     & 1932251.0  &  & \textbf{2023093}   & 2020209.8 \\
bmcp\_4200\_4400\_0.5\_7000  & 1853677     & 1820444.4  &  & \textbf{1903515}   & 1889809.5 \\
bmcp\_4400\_4200\_0.3\_10000 & 1833465     & 1816879.1  &  & \textbf{1920418}   & 1911396.2 \\
bmcp\_4400\_4200\_0.5\_7000  & 1746064     & 1730783.9  &  & \textbf{1810031}   & 1805200.7 \\
bmcp\_4400\_4400\_0.3\_10000 & 1945218     & 1922134.2  &  & \textbf{2027801}   & 2024036.1 \\
bmcp\_4400\_4400\_0.5\_7000  & 1844031     & 1821467.8  &  & \textbf{1901941}   & 1888300.5 \\
bmcp\_4400\_4600\_0.3\_10000 & 2003959     & 1993946.2  &  & \textbf{2100925}   & 2093610.1 \\
bmcp\_4400\_4600\_0.5\_7000  & 1937066     & 1906956.1  &  & \textbf{1989582}   & 1979416.6 \\
bmcp\_4600\_4400\_0.3\_10000 & 1930498     & 1913501.0  &  & \textbf{2008258}   & 2001368.8 \\
bmcp\_4600\_4400\_0.5\_7000  & 1845046     & 1817697.2  &  & \textbf{1898602}   & 1889658.5 \\
bmcp\_4600\_4600\_0.3\_10000 & 2027132     & 2005096.7  &  & \textbf{2106938}   & 2100124.5 \\
bmcp\_4600\_4600\_0.5\_7000  & 1921261     & 1900376.3  &  & \textbf{1980462}   & 1973677.2 \\
bmcp\_4600\_4800\_0.3\_10000 & 2120120     & 2091722.5  &  & \textbf{2201977}   & 2197572.4 \\
bmcp\_4600\_4800\_0.5\_7000  & 1989454     & 1967943.3  &  & \textbf{2070913}   & 2057914.3 \\
bmcp\_4800\_4600\_0.3\_10000 & 2019033     & 1991673.5  &  & \textbf{2096747}   & 2087482.0 \\
bmcp\_4800\_4600\_0.5\_7000  & 1922466     & 1901157.6  &  & \textbf{1991409}   & 1973721.9 \\
bmcp\_4800\_4800\_0.3\_10000 & 2100773     & 2058921.6  &  & \textbf{2183525}   & 2175464.8 \\
bmcp\_4800\_4800\_0.5\_7000  & 2009129     & 1973993.6  &  & \textbf{2066487}   & 2059458.7 \\
bmcp\_4800\_5000\_0.3\_10000 & 2184445     & 2157793.0  &  & \textbf{2280317}   & 2273869.0 \\
bmcp\_4800\_5000\_0.5\_7000  & 2087596     & 2050741.0  &  & \textbf{2146413}   & 2136313.2 \\
bmcp\_5000\_4800\_0.3\_10000 & 2069979     & 2051607.2  &  & \textbf{2183483}   & 2175171.2 \\
bmcp\_5000\_4800\_0.5\_7000  & 2013921     & 1977310.7  &  & \textbf{2066000}   & 2053359.9 \\
bmcp\_5000\_5000\_0.3\_10000 & 2144223     & 2126462.9  &  & \textbf{2261620}   & 2251527.0 \\
bmcp\_5000\_5000\_0.5\_7000  & 2067188     & 2046886.5  &  & \textbf{2151921}   & 2141828.6 \\
bmcp\_5000\_5200\_0.3\_10000 & 2231359     & 2220887.2  &  & \textbf{2354408}   & 2345758.7 \\
bmcp\_5000\_5200\_0.5\_7000  & 2129556     & 2115338.3  &  & \textbf{2222169}   & 2211650.9 \\ \hline
Average                      & 1967745.0   & 1943665.3  &  & \textbf{2042027.0} & 2033356.7 \\ \bottomrule
\end{tabular}}
\end{table}

==> tables/table_para.tex <==
\begin{table}[t]
\centering
\caption{\textcolor{blue}{Comparison of VDLS with different settings of parameters with 10 or 30 minutes of time limit in solving the 30 instances of the first set. Regions of the parameters are $d \in [5,10]$ and $k \in [5,10]$. Results are expressed by the average value of the best solutions of all the 30 instances obtained by the algorithms in 10 runs. Best results appear in bold.}}
\label{table_para}
\begin{tabular}{lrrrrrr} \toprule
       & $k=5$            & $k=6$            & $k=7$            & $k=8$            & $k=9$            & $k=10$  \\ \hline
\multicolumn{7}{l}{10 minutes of time limit}                                                                    \\ \hline
$d=5$  & 92191.2          & 92178.4          & 92174.3          & 92180.6          & 92178.1          & 92211.0 \\
$d=6$  & 92180.8          & 92219.7          & 92258.8          & 92249.2          & 92241.6          & 92264.6 \\
$d=7$  & 92243.1          & 92257.5          & 92254.7          & \textbf{92290.5} & 92272.6          & 92264.4 \\
$d=8$  & \textbf{92290.5} & \textbf{92290.5} & \textbf{92290.5} & 92270.9          & 92273.7          & 92222.0 \\
$d=9$  & 92280.9          & 92252.1          & 92173.4          & 92106.3          & 91985.0          & 91905.2 \\
$d=10$ & 92286.1          & 92173.3          & 92009.0          & 91925.7          & 91843.6          & 91744.3 \\ \hline
\multicolumn{7}{l}{30 minutes of time limit}                                                                    \\ \hline
$d=5$  & 92191.2          & 92178.4          & 92174.3          & 92180.6          & 92178.1          & 92211.0 \\
$d=6$  & 92180.8          & 92219.7          & 92258.8          & 92249.2          & 92241.6          & 92264.6 \\
$d=7$  & 92243.1          & 92257.5          & 92254.7          & \textbf{92290.5} & \textbf{92290.5} & 92277.3 \\
$d=8$  & \textbf{92290.5} & \textbf{92290.5} & \textbf{92290.5} & \textbf{92290.5} & \textbf{92290.5} & 92290.1 \\
$d=9$  & \textbf{92290.5} & 92268.1          & 92268.4          & 92243.1          & 92184.4          & 92109.7 \\
$d=10$ & \textbf{92290.5} & 92271.4          & 92206.0          & 92109.0          & 92016.8          & 91929.8 \\ \bottomrule
\end{tabular}
\end{table}

==> tables/table_v1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\caption{Comparison of the VDLS and its variant algorithms, VDLS$_{full}$ and VDLS$_{random}$, with 30 minutes of time limit in solving the 30 instances of the first set. Best results appear in bold.}
\label{table_v1}
\scalebox{0.65}{\begin{tabular}{lrrrrrrrr} \toprule
\multirow{2}{*}{instances}    & \multicolumn{2}{r}{VDLS$_{full}$} &  & \multicolumn{2}{r}{VDLS$_{random}$} &  & \multicolumn{2}{r}{VDLS}    \\ \cline{2-3} \cline{5-6} \cline{8-9} 
                              & best                & average     &  & best                & average       &  & best             & average  \\ \hline
bmcp\_585\_600\_0.05\_2000    & \textbf{71102}      & 71054.7     &  & 70752               & 70639.4       &  & \textbf{71102}   & 71034.4  \\
bmcp\_585\_600\_0.075\_1500   & \textbf{71025}      & 70671.5     &  & \textbf{71025}      & 70385.3       &  & \textbf{71025}   & 70492.5  \\
bmcp\_600\_585\_0.05\_2000    & \textbf{67636}      & 67636.0     &  & \textbf{67636}      & 67575.5       &  & \textbf{67636}   & 67621.6  \\
bmcp\_600\_585\_0.075\_1500   & \textbf{70588}      & 70353.0     &  & 70362               & 69900.9       &  & \textbf{70588}   & 70277.0  \\
bmcp\_600\_600\_0.05\_2000    & \textbf{68738}      & 68608.9     &  & 68387               & 68084.2       &  & \textbf{68738}   & 68580.7  \\
bmcp\_600\_600\_0.075\_1500   & \textbf{71904}      & 71780.1     &  & \textbf{71904}      & 71615.0       &  & \textbf{71904}   & 71780.7  \\
bmcp\_685\_700\_0.05\_2000    & \textbf{81227}      & 80538.2     &  & 79879               & 79852.2       &  & \textbf{81227}   & 80482.5  \\
bmcp\_685\_700\_0.075\_1500   & \textbf{83286}      & 82985.2     &  & 82931               & 82578.8       &  & \textbf{83286}   & 82886.6  \\
bmcp\_700\_685\_0.05\_2000    & \textbf{78054}      & 77751.9     &  & 77399               & 77066.5       &  & \textbf{78054}   & 77742.9  \\
bmcp\_700\_685\_0.075\_1500   & \textbf{78869}      & 78473.4     &  & 78232               & 77700.2       &  & \textbf{78869}   & 78642.9  \\
bmcp\_700\_700\_0.05\_2000    & \textbf{78458}      & 78272.6     &  & 78023               & 77488.9       &  & \textbf{78458}   & 78200.7  \\
bmcp\_700\_700\_0.075\_1500   & \textbf{84576}      & 84576.0     &  & \textbf{84576}      & 84204.3       &  & \textbf{84576}   & 84576.0  \\
bmcp\_785\_800\_0.05\_2000    & \textbf{92740}      & 92532.2     &  & \textbf{92740}      & 92141.5       &  & \textbf{92740}   & 92419.7  \\
bmcp\_785\_800\_0.075\_1500   & \textbf{95221}      & 95221.0     &  & \textbf{95221}      & 95116.5       &  & \textbf{95221}   & 95221.0  \\
bmcp\_800\_785\_0.05\_2000    & \textbf{89138}      & 89079.4     &  & 89084               & 88503.9       &  & \textbf{89138}   & 89054.7  \\
bmcp\_800\_785\_0.075\_1500   & \textbf{91856}      & 91723.8     &  & 91567               & 91006.4       &  & \textbf{91856}   & 91722.9  \\
bmcp\_800\_800\_0.05\_2000    & \textbf{91795}      & 91676.3     &  & 91443               & 90774.7       &  & \textbf{91795}   & 91604.5  \\
bmcp\_800\_800\_0.075\_1500   & \textbf{95995}      & 95590.8     &  & 95079               & 94903.0       &  & \textbf{95995}   & 95568.5  \\
bmcp\_885\_900\_0.05\_2000    & \textbf{102277}     & 102131.9    &  & 101398              & 100864.9      &  & \textbf{102277}  & 102059.2 \\
bmcp\_885\_900\_0.075\_1500   & \textbf{106940}     & 106529.1    &  & 106151              & 105876.7      &  & \textbf{106940}  & 106446.9 \\
bmcp\_900\_885\_0.05\_2000    & \textbf{99590}      & 99404.4     &  & 98680               & 98570.0       &  & \textbf{99590}   & 99368.7  \\
bmcp\_900\_885\_0.075\_1500   & \textbf{105141}     & 104991.6    &  & 104643              & 104248.2      &  & \textbf{105141}  & 105024.8 \\
bmcp\_900\_900\_0.05\_2000    & 101582              & 101185.0    &  & 100584              & 99787.1       &  & \textbf{102055}  & 101481.4 \\
bmcp\_900\_900\_0.075\_1500   & \textbf{105081}     & 104828.7    &  & 104211              & 103871.0      &  & \textbf{105081}  & 104919.1 \\
bmcp\_985\_1000\_0.05\_2000   & 110228              & 109700.8    &  & 109332              & 108917.7      &  & \textbf{110669}  & 109792.6 \\
bmcp\_985\_1000\_0.075\_1500  & \textbf{115505}     & 114977.6    &  & 114315              & 113877.7      &  & \textbf{115505}  & 114765.3 \\
bmcp\_1000\_985\_0.05\_2000   & \textbf{112057}     & 111768.8    &  & 111482              & 110461.2      &  & \textbf{112057}  & 111624.7 \\
bmcp\_1000\_985\_0.075\_1500  & \textbf{113615}     & 113153.5    &  & 112396              & 111992.6      &  & \textbf{113615}  & 113096.1 \\
bmcp\_1000\_1000\_0.05\_2000  & \textbf{113331}     & 113120.6    &  & 112893              & 112407.7      &  & \textbf{113331}  & 113129.6 \\
bmcp\_1000\_1000\_0.075\_1500 & \textbf{120246}     & 119954.1    &  & 119301              & 118994.4      &  & \textbf{120246}  & 119994.5 \\ \hline
Average                       & 92260.0             & 92009.0     &  & 91720.9             & 91313.5       &  & \textbf{92290.5} & 91987.1 
 \\ \bottomrule
\end{tabular}}
\end{table}

==> tables/table_v2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!t]
\centering
\caption{Comparison of the VDLS and its variant algorithms, VDLS$_{full}$ and VDLS$_{random}$, with 30 minutes of time limit in solving the 30 instances of the second set. Best results appear in bold.}
\label{table_v2}
\scalebox{0.6}{\begin{tabular}{lrrrrrrrr} \toprule
\multirow{2}{*}{instances}  & \multicolumn{2}{r}{VDLS$_{full}$} &  & \multicolumn{2}{r}{VDLS$_{random}$} &  & \multicolumn{2}{r}{VDLS}     \\ \cline{2-3} \cline{5-6} \cline{8-9} 
                            & best                & average     &  & best             & average          &  & best              & average  \\ \hline
bmcp\_1100\_1000\_0.3\_3000 & \textbf{143475}     & 143048.1    &  & 141054           & 141054.0         &  & \textbf{143475}   & 143224.6 \\
bmcp\_1100\_1000\_0.5\_2000 & \textbf{127157}     & 126397.4    &  & 125223           & 125223.0         &  & 126917            & 126021.6 \\
bmcp\_1100\_1100\_0.3\_3000 & \textbf{157530}     & 156853.9    &  & 155669           & 155669.0         &  & \textbf{157530}   & 156462.5 \\
bmcp\_1100\_1100\_0.5\_2000 & \textbf{139141}     & 138861.0    &  & 135927           & 135220.5         &  & \textbf{139141}   & 138719.4 \\
bmcp\_1100\_1200\_0.3\_3000 & \textbf{172660}     & 171970.2    &  & 170981           & 169663.5         &  & \textbf{172660}   & 172075.3 \\
bmcp\_1100\_1200\_0.5\_2000 & \textbf{150493}     & 149742.0    &  & 147141           & 146614.1         &  & \textbf{150493}   & 149944.0 \\
bmcp\_1200\_1100\_0.3\_3000 & \textbf{161848}     & 161832.0    &  & 161640           & 160747.3         &  & \textbf{161848}   & 161848.0 \\
bmcp\_1200\_1100\_0.5\_2000 & \textbf{137700}     & 136515.4    &  & 135501           & 134691.7         &  & \textbf{137700}   & 136831.2 \\
bmcp\_1200\_1200\_0.3\_3000 & \textbf{172595}     & 172051.9    &  & 169986           & 169256.2         &  & \textbf{172595}   & 172151.8 \\
bmcp\_1200\_1200\_0.5\_2000 & \textbf{151440}     & 149296.0    &  & 148339           & 147277.5         &  & \textbf{151440}   & 149610.0 \\
bmcp\_1200\_1300\_0.3\_3000 & 184431              & 184000.4    &  & 182282           & 181571.8         &  & \textbf{186083}   & 183599.0 \\
bmcp\_1200\_1300\_0.5\_2000 & \textbf{162154}     & 161007.4    &  & 159028           & 157862.8         &  & \textbf{162154}   & 161146.9 \\
bmcp\_1300\_1200\_0.3\_3000 & 170372              & 169693.6    &  & 167575           & 167277.2         &  & \textbf{170786}   & 169724.7 \\
bmcp\_1300\_1200\_0.5\_2000 & \textbf{151402}     & 150846.1    &  & 149747           & 148738.3         &  & \textbf{151402}   & 151049.4 \\
bmcp\_1300\_1300\_0.3\_3000 & \textbf{184699}     & 183352.8    &  & 182406           & 181178.4         &  & \textbf{184699}   & 183239.0 \\
bmcp\_1300\_1300\_0.5\_2000 & \textbf{162146}     & 161351.7    &  & 160361           & 159282.4         &  & \textbf{162146}   & 161536.7 \\
bmcp\_1300\_1400\_0.3\_3000 & \textbf{199134}     & 198864.8    &  & 195811           & 194480.4         &  & \textbf{199134}   & 198889.4 \\
bmcp\_1300\_1400\_0.5\_2000 & \textbf{173954}     & 173797.5    &  & 172420           & 171367.5         &  & \textbf{173954}   & 173799.2 \\
bmcp\_1400\_1300\_0.3\_3000 & \textbf{183987}     & 183838.8    &  & 182685           & 181441.1         &  & \textbf{183987}   & 183796.3 \\
bmcp\_1400\_1300\_0.5\_2000 & \textbf{162544}     & 162407.9    &  & 160894           & 160422.0         &  & \textbf{162544}   & 162312.9 \\
bmcp\_1400\_1400\_0.3\_3000 & \textbf{200136}     & 199564.8    &  & 198789           & 196983.3         &  & \textbf{200136}   & 199616.7 \\
bmcp\_1400\_1400\_0.5\_2000 & 174737              & 173783.8    &  & 171921           & 170531.9         &  & \textbf{175583}   & 173984.9 \\
bmcp\_1400\_1500\_0.3\_3000 & 212221              & 211189.7    &  & 211156           & 208591.6         &  & \textbf{212492}   & 211264.4 \\
bmcp\_1400\_1500\_0.5\_2000 & \textbf{186818}     & 186332.1    &  & 185133           & 184300.0         &  & \textbf{186818}   & 186250.3 \\
bmcp\_1500\_1400\_0.3\_3000 & 197184              & 196639.3    &  & 195348           & 194293.1         &  & \textbf{197219}   & 196703.4 \\
bmcp\_1500\_1400\_0.5\_2000 & \textbf{174370}     & 173451.4    &  & 171763           & 171206.7         &  & 174284            & 173576.4 \\
bmcp\_1500\_1500\_0.3\_3000 & \textbf{211108}     & 210512.8    &  & 209275           & 207887.5         &  & \textbf{211108}   & 210393.7 \\
bmcp\_1500\_1500\_0.5\_2000 & \textbf{187052}     & 185793.0    &  & 185015           & 183905.1         &  & \textbf{187052}   & 185221.6 \\
bmcp\_1500\_1600\_0.3\_3000 & \textbf{226408}     & 224819.5    &  & 223377           & 222280.0         &  & \textbf{226408}   & 224926.6 \\
bmcp\_1500\_1600\_0.5\_2000 & 198672              & 198259.5    &  & 196923           & 196291.1         &  & \textbf{199678}   & 198462.6 \\ \hline
Average                     & 173918.9            & 173202.5    &  & 171779.0         & 170843.6         &  & \textbf{174048.9} & 173212.8
 \\ \bottomrule \vspace{-2em}
\end{tabular}}
\end{table}

==> tables/table_v3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\caption{Comparison of the VDLS and its variant algorithms, VDLS$_{full}$ and VDLS$_{random}$, with 30 minutes of time limit in solving the 30 instances of the third set. Best results appear in bold.}
\label{table_v3}
\scalebox{0.56}{\begin{tabular}{lrrrrrrrr} \toprule
\multirow{2}{*}{instances}   & \multicolumn{2}{r}{VDLS$_{full}$} &  & \multicolumn{2}{r}{VDLS$_{random}$} &  & \multicolumn{2}{r}{VDLS}       \\ \cline{2-3} \cline{5-6} \cline{8-9} 
                             & best                & average     &  & best             & average          &  & best               & average   \\ \hline
bmcp\_4200\_4000\_0.3\_10000 & \textbf{1835947}    & 1829767.7   &  & 1799099          & 1793354.4        &  & \textbf{1835947}   & 1833108.2 \\
bmcp\_4200\_4000\_0.5\_7000  & 1733215             & 1725738.5   &  & 1701194          & 1696877.0        &  & \textbf{1738553}   & 1729188.0 \\
bmcp\_4200\_4200\_0.3\_10000 & 1923952             & 1918736.4   &  & 1892754          & 1890927.2        &  & \textbf{1925706}   & 1918624.2 \\
bmcp\_4200\_4200\_0.5\_7000  & 1809058             & 1803212.4   &  & 1779127          & 1777656.9        &  & \textbf{1811649}   & 1801880.2 \\
bmcp\_4200\_4400\_0.3\_10000 & 2022834             & 2020204.0   &  & 2002056          & 1997189.7        &  & \textbf{2023093}   & 2020209.8 \\
bmcp\_4200\_4400\_0.5\_7000  & 1897776             & 1888715.3   &  & 1870362          & 1863878.0        &  & \textbf{1903515}   & 1889809.5 \\
bmcp\_4400\_4200\_0.3\_10000 & 1917530             & 1908724.7   &  & 1890371          & 1885678.4        &  & \textbf{1920418}   & 1911396.2 \\
bmcp\_4400\_4200\_0.5\_7000  & 1808313             & 1804231.2   &  & 1791317          & 1788369.0        &  & \textbf{1810031}   & 1805200.7 \\
bmcp\_4400\_4400\_0.3\_10000 & \textbf{2027801}    & 2022493.1   &  & 1998685          & 1997515.4        &  & \textbf{2027801}   & 2024036.1 \\
bmcp\_4400\_4400\_0.5\_7000  & 1890349             & 1884896.0   &  & 1849547          & 1847377.2        &  & \textbf{1901941}   & 1888300.5 \\
bmcp\_4400\_4600\_0.3\_10000 & 2097111             & 2091973.3   &  & 2070880          & 2067927.9        &  & \textbf{2100925}   & 2093610.1 \\
bmcp\_4400\_4600\_0.5\_7000  & 1981566             & 1976728.2   &  & 1968883          & 1966526.8        &  & \textbf{1989582}   & 1979416.6 \\
bmcp\_4600\_4400\_0.3\_10000 & 2007323             & 2002213.2   &  & 1975158          & 1969241.9        &  & \textbf{2008258}   & 2001368.8 \\
bmcp\_4600\_4400\_0.5\_7000  & 1889059             & 1886725.1   &  & 1880145          & 1880145.0        &  & \textbf{1898602}   & 1889658.5 \\
bmcp\_4600\_4600\_0.3\_10000 & 2103993             & 2097677.7   &  & 2080601          & 2065594.8        &  & \textbf{2106938}   & 2100124.5 \\
bmcp\_4600\_4600\_0.5\_7000  & 1978206             & 1972638.7   &  & 1953721          & 1953251.9        &  & \textbf{1980462}   & 1973677.2 \\
bmcp\_4600\_4800\_0.3\_10000 & \textbf{2201977}    & 2197678.1   &  & 2171744          & 2171497.4        &  & \textbf{2201977}   & 2197572.4 \\
bmcp\_4600\_4800\_0.5\_7000  & 2069048             & 2058651.2   &  & 2039254          & 2036251.6        &  & \textbf{2070913}   & 2057914.3 \\
bmcp\_4800\_4600\_0.3\_10000 & 2091456             & 2084178.6   &  & 2055984          & 2055318.2        &  & \textbf{2096747}   & 2087482.0 \\
bmcp\_4800\_4600\_0.5\_7000  & 1980482             & 1971733.9   &  & 1937401          & 1937401.0        &  & \textbf{1991409}   & 1973721.9 \\
bmcp\_4800\_4800\_0.3\_10000 & 2181967             & 2171730.1   &  & 2151323          & 2143758.3        &  & \textbf{2183525}   & 2175464.8 \\
bmcp\_4800\_4800\_0.5\_7000  & 2064768             & 2058002.9   &  & 2029868          & 2029556.6        &  & \textbf{2066487}   & 2059458.7 \\
bmcp\_4800\_5000\_0.3\_10000 & 2278226             & 2273093.1   &  & 2261424          & 2261424.0        &  & \textbf{2280317}   & 2273869.0 \\
bmcp\_4800\_5000\_0.5\_7000  & 2140951             & 2133532.0   &  & 2110025          & 2110025.0        &  & \textbf{2146413}   & 2136313.2 \\
bmcp\_5000\_4800\_0.3\_10000 & 2183270             & 2174154.3   &  & 2144805          & 2135011.9        &  & \textbf{2183483}   & 2175171.2 \\
bmcp\_5000\_4800\_0.5\_7000  & 2064436             & 2053364.9   &  & 2036595          & 2036595.0        &  & \textbf{2066000}   & 2053359.9 \\
bmcp\_5000\_5000\_0.3\_10000 & 2257921             & 2250425.2   &  & 2232094          & 2222644.0        &  & \textbf{2261620}   & 2251527.0 \\
bmcp\_5000\_5000\_0.5\_7000  & 2145398             & 2140167.1   &  & 2119843          & 2119843.0        &  & \textbf{2151921}   & 2141828.6 \\
bmcp\_5000\_5200\_0.3\_10000 & 2352860             & 2345247.5   &  & 2313592          & 2310718.3        &  & \textbf{2354408}   & 2345758.7 \\
bmcp\_5000\_5200\_0.5\_7000  & 2214566             & 2208215.9   &  & 2193299          & 2191433.5        &  & \textbf{2222169}   & 2211650.9 \\ \hline
Average                      & 2038378.6           & 2031828.3   &  & 2010038.4        & 2006766.3        &  & \textbf{2042027.0} & 2033356.7 \\ \bottomrule \vspace{-2.5em}
\end{tabular}}
\end{table}

==> tables/table_v4.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\caption{Comparison of the VDLS and its variant algorithms, VDLS$_{empty\_init}$ and VDLS$_{random\_init}$, as well as the PLTS algorithm, with 30 minutes of time limit in solving the 30 instances of the first set. Best results appear in bold.}
\label{table_v4}
\scalebox{0.6}{\begin{tabular}{lrrrrrrrrrrr} \toprule
\multirow{2}{*}{Instances}    & \multicolumn{2}{r}{PLTS}   &  & \multicolumn{2}{r}{VDLS$_{empty\_init}$} &  & \multicolumn{2}{r}{VDLS$_{random\_init}$} &  & \multicolumn{2}{r}{VDLS}    \\ \cline{2-3} \cline{5-6} \cline{8-9} \cline{11-12} 
                              & best            & average  &  & best                   & average         &  & best                    & average         &  & best             & average  \\ \hline
bmcp\_585\_600\_0.05\_2000    & \textbf{71102}  & 70915.0  &  & \textbf{71102}         & 71013.3         &  & \textbf{71102}          & 71021.2         &  & \textbf{71102}   & 71034.4  \\
bmcp\_585\_600\_0.075\_1500   & 70677           & 70670.2  &  & \textbf{71025}         & 70472.0         &  & \textbf{71025}          & 70455.0         &  & \textbf{71025}   & 70492.5  \\
bmcp\_600\_585\_0.05\_2000    & \textbf{67636}  & 67041.5  &  & \textbf{67636}         & 67588.8         &  & \textbf{67636}          & 67621.6         &  & \textbf{67636}   & 67621.6  \\
bmcp\_600\_585\_0.075\_1500   & 70318           & 70318.0  &  & \textbf{70588}         & 70155.1         &  & \textbf{70588}          & 70192.9         &  & \textbf{70588}   & 70277.0  \\
bmcp\_600\_600\_0.05\_2000    & 68453           & 68386.8  &  & \textbf{68738}         & 68521.4         &  & 68634                   & 68512.1         &  & \textbf{68738}   & 68580.7  \\
bmcp\_600\_600\_0.075\_1500   & 71746           & 71746.0  &  & \textbf{71904}         & 71720.3         &  & \textbf{71904}          & 71730.3         &  & \textbf{71904}   & 71780.7  \\
bmcp\_685\_700\_0.05\_2000    & 80197           & 80096.6  &  & \textbf{81227}         & 80934.6         &  & \textbf{81227}          & 81009.0         &  & \textbf{81227}   & 80482.5  \\
bmcp\_685\_700\_0.075\_1500   & 82955           & 82944.2  &  & 82955                  & 82823.8         &  & \textbf{83286}          & 82840.5         &  & \textbf{83286}   & 82886.6  \\
bmcp\_700\_685\_0.05\_2000    & 77876           & 77372.7  &  & \textbf{78054}         & 77915.0         &  & \textbf{78054}          & 77760.8         &  & \textbf{78054}   & 77742.9  \\
bmcp\_700\_685\_0.075\_1500   & \textbf{78869}  & 78810.4  &  & \textbf{78869}         & 78759.3         &  & \textbf{78869}          & 78547.3         &  & \textbf{78869}   & 78642.9  \\
bmcp\_700\_700\_0.05\_2000    & 78028           & 77501.5  &  & \textbf{78458}         & 78181.1         &  & \textbf{78458}          & 78238.8         &  & \textbf{78458}   & 78200.7  \\
bmcp\_700\_700\_0.075\_1500   & 84570           & 83720.7  &  & \textbf{84576}         & 84576.0         &  & \textbf{84576}          & 84576.0         &  & \textbf{84576}   & 84576.0  \\
bmcp\_785\_800\_0.05\_2000    & 92431           & 92195.7  &  & 92608                  & 92477.3         &  & 92608                   & 92339.7         &  & \textbf{92740}   & 92419.7  \\
bmcp\_785\_800\_0.075\_1500   & 94245           & 94245.0  &  & \textbf{95221}         & 94466.1         &  & \textbf{95221}          & 94641.6         &  & \textbf{95221}   & 95221.0  \\
bmcp\_800\_785\_0.05\_2000    & 88562           & 88560.3  &  & \textbf{89138}         & 88911.4         &  & \textbf{89138}          & 89049.4         &  & \textbf{89138}   & 89054.7  \\
bmcp\_800\_785\_0.075\_1500   & 91021           & 90971.8  &  & \textbf{91856}         & 91435.5         &  & \textbf{91856}          & 91320.7         &  & \textbf{91856}   & 91722.9  \\
bmcp\_800\_800\_0.05\_2000    & 91748           & 90934.2  &  & \textbf{91795}         & 91686.4         &  & \textbf{91795}          & 91446.4         &  & \textbf{91795}   & 91604.5  \\
bmcp\_800\_800\_0.075\_1500   & 95533           & 95533.0  &  & 95746                  & 95298.2         &  & \textbf{95995}          & 95340.6         &  & \textbf{95995}   & 95568.5  \\
bmcp\_885\_900\_0.05\_2000    & 101293          & 101142.0 &  & \textbf{102277}        & 102031.0        &  & \textbf{102277}         & 102049.7        &  & \textbf{102277}  & 102059.2 \\
bmcp\_885\_900\_0.075\_1500   & 106364          & 105782.6 &  & \textbf{106940}        & 106719.6        &  & \textbf{106940}         & 106618.8        &  & \textbf{106940}  & 106446.9 \\
bmcp\_900\_885\_0.05\_2000    & 98840           & 98645.4  &  & \textbf{99590}         & 99203.7         &  & \textbf{99590}          & 99304.8         &  & \textbf{99590}   & 99368.7  \\
bmcp\_900\_885\_0.075\_1500   & \textbf{105141} & 103846.9 &  & \textbf{105141}        & 105091.2        &  & \textbf{105141}         & 105041.4        &  & \textbf{105141}  & 105024.8 \\
bmcp\_900\_900\_0.05\_2000    & 101265          & 101211.4 &  & \textbf{102055}        & 101366.5        &  & \textbf{102055}         & 101467.8        &  & \textbf{102055}  & 101481.4 \\
bmcp\_900\_900\_0.075\_1500   & 104521          & 104521.0 &  & \textbf{105081}        & 104642.9        &  & \textbf{105081}         & 104629.0        &  & \textbf{105081}  & 104919.1 \\
bmcp\_985\_1000\_0.05\_2000   & 109567          & 108938.0 &  & \textbf{110669}        & 109936.4        &  & \textbf{110669}         & 110095.6        &  & \textbf{110669}  & 109792.6 \\
bmcp\_985\_1000\_0.075\_1500  & 113541          & 113541.0 &  & \textbf{115505}        & 114943.2        &  & \textbf{115505}         & 115188.6        &  & \textbf{115505}  & 114765.3 \\
bmcp\_1000\_985\_0.05\_2000   & 111176          & 110712.6 &  & \textbf{112057}        & 111854.8        &  & \textbf{112057}         & 111570.4        &  & \textbf{112057}  & 111624.7 \\
bmcp\_1000\_985\_0.075\_1500  & 112250          & 112218.9 &  & \textbf{113615}        & 113021.8        &  & \textbf{113615}         & 112743.9        &  & \textbf{113615}  & 113096.1 \\
bmcp\_1000\_1000\_0.05\_2000  & 112640          & 111577.8 &  & \textbf{113331}        & 113165.4        &  & \textbf{113331}         & 113140.3        &  & \textbf{113331}  & 113129.6 \\
bmcp\_1000\_1000\_0.075\_1500 & 119453          & 118499.3 &  & \textbf{120246}        & 119660.3        &  & \textbf{120246}         & 119913.0        &  & \textbf{120246}  & 119994.5 \\ \hline
Average                       & 91733.9         & 91420.0  &  & 92266.8                & 91952.4         &  & 92282.6                 & 91946.9         &  & \textbf{92290.5} & 91987.1 
 \\ \bottomrule
\end{tabular}}
\end{table}

==> tables/table_v5.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!t]
\centering
\caption{Comparison of the VDLS and its variant algorithms, VDLS$_{empty\_init}$ and VDLS$_{random\_init}$, as well as the PLTS algorithm, with 30 minutes of time limit in solving the 30 instances of the second set. Best results appear in bold.}
\label{table_v5}
\scalebox{0.6}{\begin{tabular}{lrrrrrrrrrrr} \toprule
\multirow{2}{*}{Instances}  & \multicolumn{2}{r}{PLTS}   &  & \multicolumn{2}{r}{VDLS$_{empty\_init}$} &  & \multicolumn{2}{r}{VDLS$_{random\_init}$} &  & \multicolumn{2}{r}{VDLS}     \\ \cline{2-3} \cline{5-6} \cline{8-9} \cline{11-12} 
                            & best            & average  &  & best                   & average         &  & best                    & average         &  & best              & average  \\ \hline
bmcp\_1100\_1000\_0.3\_3000 & 142835          & 142428.7 &  & \textbf{143475}        & 143052.0        &  & \textbf{143475}         & 143317.0        &  & \textbf{143475}   & 143224.6 \\
bmcp\_1100\_1000\_0.5\_2000 & 125974          & 125790.0 &  & \textbf{127157}        & 126628.5        &  & 126792                  & 126400.0        &  & 126917            & 126021.6 \\
bmcp\_1100\_1100\_0.3\_3000 & 154936          & 154661.7 &  & \textbf{157530}        & 156913.1        &  & 157264                  & 156684.0        &  & \textbf{157530}   & 156462.5 \\
bmcp\_1100\_1100\_0.5\_2000 & \textbf{139196} & 138169.0 &  & \textbf{139196}        & 138470.8        &  & \textbf{139196}         & 138679.7        &  & 139141            & 138719.4 \\
bmcp\_1100\_1200\_0.3\_3000 & 169113          & 168763.6 &  & \textbf{172660}        & 172348.5        &  & \textbf{172660}         & 172137.0        &  & \textbf{172660}   & 172075.3 \\
bmcp\_1100\_1200\_0.5\_2000 & 150301          & 149366.4 &  & \textbf{150493}        & 149920.9        &  & \textbf{150493}         & 150039.2        &  & \textbf{150493}   & 149944.0 \\
bmcp\_1200\_1100\_0.3\_3000 & \textbf{161848} & 159620.3 &  & \textbf{161848}        & 161848.0        &  & \textbf{161848}         & 161848.0        &  & \textbf{161848}   & 161848.0 \\
bmcp\_1200\_1100\_0.5\_2000 & 135858          & 135509.2 &  & 137046                 & 136658.3        &  & 136995                  & 136380.8        &  & \textbf{137700}   & 136831.2 \\
bmcp\_1200\_1200\_0.3\_3000 & 169219          & 168821.7 &  & \textbf{172595}        & 172238.3        &  & \textbf{172595}         & 172154.5        &  & \textbf{172595}   & 172151.8 \\
bmcp\_1200\_1200\_0.5\_2000 & 149654          & 148679.1 &  & \textbf{151440}        & 149839.0        &  & \textbf{151440}         & 149991.3        &  & \textbf{151440}   & 149610.0 \\
bmcp\_1200\_1300\_0.3\_3000 & 183004          & 182220.4 &  & 184384                 & 183829.5        &  & 184195                  & 183609.9        &  & \textbf{186083}   & 183599.0 \\
bmcp\_1200\_1300\_0.5\_2000 & 160369          & 159735.4 &  & \textbf{162154}        & 161180.2        &  & \textbf{162154}         & 161188.3        &  & \textbf{162154}   & 161146.9 \\
bmcp\_1300\_1200\_0.3\_3000 & 168586          & 168473.8 &  & 170283                 & 169933.0        &  & \textbf{170786}         & 169874.1        &  & \textbf{170786}   & 169724.7 \\
bmcp\_1300\_1200\_0.5\_2000 & 151067          & 150034.7 &  & 151402                 & 150650.5        &  & \textbf{151512}         & 150982.9        &  & 151402            & 151049.4 \\
bmcp\_1300\_1300\_0.3\_3000 & 180608          & 179978.4 &  & \textbf{184699}        & 183104.5        &  & 184627                  & 183237.6        &  & \textbf{184699}   & 183239.0 \\
bmcp\_1300\_1300\_0.5\_2000 & 160485          & 159511.3 &  & \textbf{162146}        & 161168.5        &  & \textbf{162146}         & 160950.0        &  & \textbf{162146}   & 161536.7 \\
bmcp\_1300\_1400\_0.3\_3000 & 197709          & 195681.9 &  & \textbf{199134}        & 198992.4        &  & \textbf{199134}         & 198914.6        &  & \textbf{199134}   & 198889.4 \\
bmcp\_1300\_1400\_0.5\_2000 & 173349          & 171665.0 &  & \textbf{173954}        & 173445.6        &  & \textbf{173954}         & 173559.3        &  & \textbf{173954}   & 173799.2 \\
bmcp\_1400\_1300\_0.3\_3000 & 182881          & 180143.5 &  & \textbf{183987}        & 183465.6        &  & 183914                  & 183677.0        &  & \textbf{183987}   & 183796.3 \\
bmcp\_1400\_1300\_0.5\_2000 & 161995          & 160647.0 &  & 162446                 & 161748.9        &  & 162465                  & 161986.3        &  & \textbf{162544}   & 162312.9 \\
bmcp\_1400\_1400\_0.3\_3000 & 199879          & 197229.0 &  & \textbf{200136}        & 199469.9        &  & \textbf{200136}         & 199824.5        &  & \textbf{200136}   & 199616.7 \\
bmcp\_1400\_1400\_0.5\_2000 & 174683          & 173393.1 &  & \textbf{175583}        & 174009.4        &  & 174683                  & 173992.4        &  & \textbf{175583}   & 173984.9 \\
bmcp\_1400\_1500\_0.3\_3000 & 210077          & 208315.6 &  & 212267                 & 211120.3        &  & 211494                  & 211274.1        &  & \textbf{212492}   & 211264.4 \\
bmcp\_1400\_1500\_0.5\_2000 & 184259          & 183289.9 &  & 185902                 & 185071.3        &  & 186619                  & 184816.6        &  & \textbf{186818}   & 186250.3 \\
bmcp\_1500\_1400\_0.3\_3000 & 194156          & 193554.8 &  & \textbf{197219}        & 196694.9        &  & \textbf{197219}         & 196650.0        &  & \textbf{197219}   & 196703.4 \\
bmcp\_1500\_1400\_0.5\_2000 & 173475          & 171426.9 &  & \textbf{174284}        & 173810.6        &  & \textbf{174284}         & 173953.5        &  & \textbf{174284}   & 173576.4 \\
bmcp\_1500\_1500\_0.3\_3000 & 209929          & 207795.3 &  & \textbf{211108}        & 210447.6        &  & \textbf{211108}         & 210857.9        &  & \textbf{211108}   & 210393.7 \\
bmcp\_1500\_1500\_0.5\_2000 & 184082          & 182676.2 &  & \textbf{187052}        & 185348.1        &  & 185931                  & 185251.3        &  & \textbf{187052}   & 185221.6 \\
bmcp\_1500\_1600\_0.3\_3000 & \textbf{226408} & 221641.3 &  & \textbf{226408}        & 224705.0        &  & \textbf{226408}         & 225218.9        &  & \textbf{226408}   & 224926.6 \\
bmcp\_1500\_1600\_0.5\_2000 & 198214          & 196659.0 &  & 198672                 & 198052.5        &  & 198834                  & 197922.9        &  & \textbf{199678}   & 198462.6 \\ \hline
Average                     & 172471.6        & 171196.1 &  & 173888.7               & 173138.9        &  & 173812.0                & 173179.1        &  & \textbf{174048.9} & 173212.8
 \\ \bottomrule \vspace{-2em}
\end{tabular}}
\end{table}

==> tables/table_v6.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\caption{Comparison of the VDLS and its variant algorithms, VDLS$_{empty\_init}$ and VDLS$_{random\_init}$, as well as the PLTS algorithm, with 30 minutes of time limit in solving the 30 instances of the third set. Best results appear in bold.}
\label{table_v6}
\scalebox{0.56}{\begin{tabular}{lrrrrrrrrrrr} \toprule
\multirow{2}{*}{Instances}   & \multicolumn{2}{r}{PLTS} &  & \multicolumn{2}{r}{VDLS$_{empty\_init}$} &  & \multicolumn{2}{r}{VDLS$_{random\_init}$} &  & \multicolumn{2}{r}{VDLS}       \\ \cline{2-3} \cline{5-6} \cline{8-9} \cline{11-12} 
                             & best        & average    &  & best                   & average         &  & best                & average             &  & best               & average   \\ \hline
bmcp\_4200\_4000\_0.3\_10000 & 1778013     & 1747411.9  &  & 1834284                & 1803563.4       &  & 1833972             & 1803414.7           &  & \textbf{1835947}   & 1833108.2 \\
bmcp\_4200\_4000\_0.5\_7000  & 1685141     & 1666673.3  &  & 1731239                & 1711775.5       &  & 1728424             & 1706506.7           &  & \textbf{1738553}   & 1729188.0 \\
bmcp\_4200\_4200\_0.3\_10000 & 1874190     & 1839780.1  &  & 1891453                & 1880097.5       &  & 1906804             & 1885572.2           &  & \textbf{1925706}   & 1918624.2 \\
bmcp\_4200\_4200\_0.5\_7000  & 1764277     & 1742121.7  &  & 1799917                & 1774357.8       &  & 1807742             & 1779957.7           &  & \textbf{1811649}   & 1801880.2 \\
bmcp\_4200\_4400\_0.3\_10000 & 1954069     & 1932251.0  &  & 1978774                & 1971898.8       &  & 1976199             & 1972521.3           &  & \textbf{2023093}   & 2020209.8 \\
bmcp\_4200\_4400\_0.5\_7000  & 1853677     & 1820444.4  &  & 1888408                & 1861994.5       &  & 1901803             & 1860441.4           &  & \textbf{1903515}   & 1889809.5 \\
bmcp\_4400\_4200\_0.3\_10000 & 1833465     & 1816879.1  &  & 1915183                & 1878661.3       &  & 1885127             & 1878187.1           &  & \textbf{1920418}   & 1911396.2 \\
bmcp\_4400\_4200\_0.5\_7000  & 1746064     & 1730783.9  &  & 1795133                & 1771581.4       &  & 1777184             & 1766877.8           &  & \textbf{1810031}   & 1805200.7 \\
bmcp\_4400\_4400\_0.3\_10000 & 1945218     & 1922134.2  &  & 2022238                & 1995933.5       &  & 1985214             & 1978845.9           &  & \textbf{2027801}   & 2024036.1 \\
bmcp\_4400\_4400\_0.5\_7000  & 1844031     & 1821467.8  &  & 1895699                & 1864656.6       &  & 1865846             & 1853948.8           &  & \textbf{1901941}   & 1888300.5 \\
bmcp\_4400\_4600\_0.3\_10000 & 2003959     & 1993946.2  &  & 2089841                & 2048418.3       &  & 2098311             & 2057479.1           &  & \textbf{2100925}   & 2093610.1 \\
bmcp\_4400\_4600\_0.5\_7000  & 1937066     & 1906956.1  &  & 1978452                & 1947386.4       &  & 1988053             & 1943530.0           &  & \textbf{1989582}   & 1979416.6 \\
bmcp\_4600\_4400\_0.3\_10000 & 1930498     & 1913501.0  &  & 1971422                & 1963026.3       &  & 1995420             & 1966461.0           &  & \textbf{2008258}   & 2001368.8 \\
bmcp\_4600\_4400\_0.5\_7000  & 1845046     & 1817697.2  &  & 1889987                & 1857307.9       &  & 1887876             & 1863836.3           &  & \textbf{1898602}   & 1889658.5 \\
bmcp\_4600\_4600\_0.3\_10000 & 2027132     & 2005096.7  &  & 2103372                & 2059542.7       &  & 2057082             & 2048803.4           &  & \textbf{2106938}   & 2100124.5 \\
bmcp\_4600\_4600\_0.5\_7000  & 1921261     & 1900376.3  &  & 1971064                & 1937988.1       &  & 1950337             & 1938807.7           &  & \textbf{1980462}   & 1973677.2 \\
bmcp\_4600\_4800\_0.3\_10000 & 2120120     & 2091722.5  &  & 2201518                & 2177117.9       &  & 2196065             & 2168175.1           &  & \textbf{2201977}   & 2197572.4 \\
bmcp\_4600\_4800\_0.5\_7000  & 1989454     & 1967943.3  &  & 2062229                & 2019898.7       &  & 2065687             & 2040861.3           &  & \textbf{2070913}   & 2057914.3 \\
bmcp\_4800\_4600\_0.3\_10000 & 2019033     & 1991673.5  &  & 2054553                & 2044674.6       &  & 2085908             & 2049130.6           &  & \textbf{2096747}   & 2087482.0 \\
bmcp\_4800\_4600\_0.5\_7000  & 1922466     & 1901157.6  &  & 1981511                & 1943407.6       &  & 1971668             & 1942246.4           &  & \textbf{1991409}   & 1973721.9 \\
bmcp\_4800\_4800\_0.3\_10000 & 2100773     & 2058921.6  &  & 2176277                & 2130880.7       &  & 2172264             & 2130106.7           &  & \textbf{2183525}   & 2175464.8 \\
bmcp\_4800\_4800\_0.5\_7000  & 2009129     & 1973993.6  &  & \textbf{2068419}       & 2038013.3       &  & 2049709             & 2022473.7           &  & 2066487            & 2059458.7 \\
bmcp\_4800\_5000\_0.3\_10000 & 2184445     & 2157793.0  &  & 2224114                & 2216495.4       &  & 2268312             & 2226567.3           &  & \textbf{2280317}   & 2273869.0 \\
bmcp\_4800\_5000\_0.5\_7000  & 2087596     & 2050741.0  &  & 2133028                & 2092000.2       &  & 2134855             & 2103473.5           &  & \textbf{2146413}   & 2136313.2 \\
bmcp\_5000\_4800\_0.3\_10000 & 2069979     & 2051607.2  &  & 2158927                & 2121501.3       &  & 2168454             & 2127542.6           &  & \textbf{2183483}   & 2175171.2 \\
bmcp\_5000\_4800\_0.5\_7000  & 2013921     & 1977310.7  &  & 2055668                & 2021525.7       &  & 2064677             & 2027452.6           &  & \textbf{2066000}   & 2053359.9 \\
bmcp\_5000\_5000\_0.3\_10000 & 2144223     & 2126462.9  &  & 2239557                & 2199620.3       &  & 2206885             & 2201582.7           &  & \textbf{2261620}   & 2251527.0 \\
bmcp\_5000\_5000\_0.5\_7000  & 2067188     & 2046886.5  &  & 2098393                & 2088820.7       &  & 2120476             & 2096355.4           &  & \textbf{2151921}   & 2141828.6 \\
bmcp\_5000\_5200\_0.3\_10000 & 2231359     & 2220887.2  &  & 2331638                & 2294991.9       &  & 2332974             & 2289507.8           &  & \textbf{2354408}   & 2345758.7 \\
bmcp\_5000\_5200\_0.5\_7000  & 2129556     & 2115338.3  &  & 2217338                & 2175089.1       &  & 2209861             & 2171932.5           &  & \textbf{2222169}   & 2211650.9 \\ \hline
Average                      & 1967745.0   & 1943665.3  &  & 2025321.2              & 1996407.6       &  & 2023106.3           & 1996753.3           &  & \textbf{2042027.0} & 2033356.7
 \\ \bottomrule \vspace{-2em}
\end{tabular}}
\end{table}
